Beyond the "Industry Standard": Focusing Gender-Affirming Voice Training Technologies on Individualized Goal Exploration

Gender-affirming voice training is critical for the transition process for many transgender individuals, enabling their voice to align with their gender identity. Individualized voice goals guide and motivate the voice training journey, but existing voice training technologies fail to define clear goals. We interviewed six voice experts and ten transgender individuals with voice training experience (voice trainees), focusing on how they defined, triangulated, and used voice goals. We found that goal voice exploration involves navigation between descriptive and technical goals, and continuous reevaluation throughout the voice training journey. Our study reveals how goal descriptions, subjective satisfaction, voice examples, and voice modification and training technologies inform goal exploration, and identifies risks of overemphasizing goals. We identified technological implications informed by existing expert and trainee strategies, and provide guidelines for supporting individualized goals throughout the voice training journey based on brainstorming with trainees and experts.

==> Figures/GVD_pipeline.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[node distance=2cm]
    % Define styles
    \tikzstyle{process} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!20]
    \tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!20]
    \tikzstyle{arrow} = [thick,->,>=stealth]

    % Nodes
    \node (start) [process] {Start};
    \node (filter) [process, below of=start] {Filter \& Arrange Models};
    \node (present) [process, below of=filter] {Present Models};
    \node (test) [process, below of=present] {Test Models};
    \node (like) [decision, below of=test, yshift=-1cm] {Like Models?};
    \node (merge) [process, right of=like, xshift=2cm] {Merge/Modify Models};
    \node (visualize) [process, below of=like, yshift=-1cm] {Visualize Journey};
    \node (accept) [decision, below of=visualize, yshift=-1cm] {Accept Journey?};
    \node (end) [process, below of=accept, yshift=-1cm] {End \& Output};

    % Arrows
    \draw [arrow] (start) -- (filter);
    \draw [arrow] (filter) -- (present);
    \draw [arrow] (present) -- (test);
    \draw [arrow] (test) -- (like);
    \draw [arrow] (like) -- node[anchor=east] {Yes} (visualize);
    \draw [arrow] (like) -- node[anchor=south] {No} (filter);
    \draw [arrow] (like) -- node[anchor=south] {Partial} (merge);
    \draw [arrow] (merge) -- (test);
    \draw [arrow] (visualize) -- (accept);
    \draw [arrow] (accept) -- node[anchor=east] {Yes} (end);
    \draw [arrow] (accept) -- node[anchor=south] {No} (filter);

    % Notes
    \node [text width=4cm, align=left, right of=filter, xshift=3cm] {
        1. Uses trainee preferences and abilities
        2. Optional: similarity to provided example
    };
    \node [text width=4cm, align=left, right of=test, xshift=3cm] {
        1. Pre-recorded phrases
        2. Real-time voice changer
    };
    \node [text width=4cm, align=left, right of=merge, xshift=3cm] {
        1. Merge multiple models
        2. Enhance with parameter-based changes
    };
    \node [text width=4cm, align=left, left of=visualize, xshift=-3cm] {
        1. Estimate journey based on survey
        2. Create "milestone" voices
    };
    \node [text width=4cm, align=left, left of=end, xshift=-3cm] {
        Output:
        1. Goal model(s)
        2. Relevant parameters
        3. Journey visualization
        4. Milestone models
    };
\end{tikzpicture}
\caption{Goal-Voice-Discovery (GVD) Tool Pipeline}
\label{fig:gvd-pipeline}
\end{figure}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> extra_files/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> extra_files/old_versions/findings.tex <==
\subsection{What is a Goal?}
\label{sec:findings:what_is_a_goal}
Previous works on voice training technologies failed to define a clear boundary between overall voice end-goals and voice targets. To better separate these two ideas, we define \textit{voice goals} as the overall heading of the voice training journey, which can be a clear point with specific parameters or characteristics, or a rough area defined through approximate voice features. We define \textit{voice targets} as the measures of success used in daily voice practice, which oftentimes are incremental. While some trainees may use voice goals as targets, experts recommend against doing so. Through focusing on voice goals, %we found that trainees and experts had various ways of defining the ideal end-point to voice training. We found that voice goals
we identified two categories of voice goals: \textit{approximate goals}, which represent the driving factors behind voice training, and \textit{clear goals}, which define a precise direction for voice training.

\subsubsection{Approximate Goals.} We found that while trainees typically didn't have the knowledge to verbalize their initial goals in terms of technical vocal parameters, they still had various characteristics in mind when defining the direction of their goals. These approximate goals embodied aspects of vocal utility, comfort, identity representation, or basic parameter explanations. While experts sought to clarify these goals through skill and knowledge-building, the technologies trainees used when training independently measured success directly using approximate goals.

% \textbf{\textit{Types of Approximate Goals}} 
% Trainees defined approximate goals in terms of utility of the voice, such as having a voice that passes (), representation of their identity, such as having a voice that better represents their gender, a need for personal satisfaction with the voice, such as a voice that doesn't cause dysphoria, or basic single-parameter explanations, such as wanting a higher or lower pitch (). 
\textbf{\textit{Vocal Utility.}} Vocal utility plays a key role in defining why a trainee initially pursues voice training. Specifically, we found that trainees wanted a voice that causes others to treat them a specific way, whether that be passing as cisgender (T1, T3, T4, T8-T10 and E1, E3, E6), causing some amount of gender confusion (T6), or presenting authority (T1, T2, T10). For example, T2 desired a voice so masculine that it would make his coworkers who misgendered him look silly. T6 wanted a voice on the threshold, where most of the time they would be gendered as male, but a small percentage of the time they would be gendered as female by others. T2 and T4 mentioned that having access to a voice that passed as cisgender would allow them to maintain safety in dangerous environments.

\textbf{\textit{Comfort in Voice.}} Trainees mentioned alleviation of voice dysphoria and gaining a voice that they felt comfortable with as a major factor driving their voice training (T1 and T9). Although providing a point to get away from (the current voice), voice dysphoria oftentimes didn't provide a very useful motivation --- instead, experts recognized voice dysphoria as a common barrier to voice training (E1, E2, E4, E5), especially when related to \textit{voice generalization}, which involves using the voice-in-training (VIT) in new environments (E1, E4, E5). E1 mentioned how voice dysphoria was a common barrier to practicing outside the session: \textit{``[They're] going home to practice, and if what comes out isn't euphoric, it can be ... a barrier to practicing at all.''} %\yuhang{quote?}%Experts

\textbf{\textit{Identity Representation.}} Identity representation through voice plays a key factor in individualizing the voice goal, providing a vague direction for voice training. Based on the experiences of trainees and experts, we found that identity-based descriptions provided different tiers of specificity. By definition, gender-affirming voice trainees seek to acquire a voice that is affirming for representing their gender identities (E3-E6). More specifically, some trainees may desire to have a voice that represents their culture or region (T2 and T10). Voice archetypes and character descriptions, such as ``pretty boy'' (T10), provide the most detailed representations of approximate goals, since they can be easily connected to examples (E1, E2, E5, E6). E2 remembered how a character described by a trainee gave her a clear idea of the voice that the trainee wanted:
\begin{quote}
    \textit{``I had one client who said that their ideal voice would be someone who could rock a ball gown but then get in a fight in a bodega. It's a very clear character of what she wanted to sound like.''}
\end{quote}

\textbf{\textit{Parameter-based Goals.}} Trainees with a general knowledge of voice may start with an end-goal focused on shifting specific vocal parameters or characteristics (T1, T2, T4, T6, T9 and E4, E6). While providing direction for voice training, this kind of approximate goal may arise from a misconception of the importance of the single parameter, which is usually pitch (T5 and T9). Experts build a healthy understanding of voice parameters among trainees, allowing trainees to better leverage parameters for approximating their voice goals (E1-E3, E4, E6)

\textbf{\textit{Approximate Goals in Voice Technologies.}} Voice training technologies like voice tools \cite{voice_tools} use gender-range-based voice targets to attach the approximate goal of presenting gender identity through voice to specific pitch ranges. Trainees and experts lamented that this consistent categorization of voice based on pitch characteristics not only misleads trainees through over-emphasizing pitch (T3, T5, T7-T9 and E1-E3, E5), but also creates unsustainable targets for practice by failing to separate target-setting from goal-setting (T1, T5, T9, T10 and E1, E2, E4, E6).

\textbf{\textit{Approximate Goals in Voice Training Media.}} While voice training media is a helpful tool for building voice training skills, the untargeted nature of media results in it pushing ideal voice ``standards'' that don't necessarily align with trainees' identities (T1, T8-T10). T9 developed a Californian ``valley girl'' accent because of the vowel training methods she learned from YouTube, resulting in others mis-identifying her as Californian. T1 described this ``industry-standard'' voice for transfemme individuals:
\begin{quote}
     \textit{``I'm not going to keep pursuing... the industry standard of `We're going to make you sound like you're AFAB. We're going to make you sound like you're 16'.''}
\end{quote}
\subsubsection{Clear Goals.} %\yuhang{the first couple of sentences read a bit like background. However, these are your findings, and you identified and defined the concept of these types of goals via your findings. Make sure that you convey that in the writing. For example, at the beginning of5.1, you can say that we identified various types of goals, including xx, xx, used by trainees or experts to achieve xxx. Or at least, to highlight something is your finding instead of some clinical background, you should say "we found that xx."}
Clear goals represent an exact direction for voice training (E1-E3, E5, E6) through providing a combination of voice characteristics for a trainee to work toward. These goals allow experts to craft individualized training regimens and provide a clearer representation of goal characteristics to voice trainees than approximate goals (E2, E5, E6). We found that experts and trainees triangulate clear goals through combinations of examples and approximate goals, setting a clear direction for voice training.

\textbf{\textit{Example-based Goals.}} Voice examples provided clear goal directions for voice training (E1-E3, E5, E6), as they directly demonstrated voice characteristics which the trainee could work towards. Voice examples used in goal voice exploration came from various aspects of trainees' lives, including people around them (e.g. friends and family) (T1-T3, T10 and E1, E2, E5), singers, voice actors, and celebrities (T1, T4, T5, T10 and E6), and online personalities, both transgender (T5, T9, T10) and cisgender (T10).  Through representing desired vocal characteristics through a single example or multiple examples, experts and trainees could both use examples directly as points of comparison (E1-E3) and indirectly through measuring vocal parameters from the example and using them for goal and target-setting (E1-E3, E5, E6).

\textbf{\textit{Combined Approximate Goals}} While singular approximate goals provide vague direction for voice goals, the combined approximation of multiple vague goals can provide a clear direction for voice training, especially with the guidance of an expert (T7, T8 and E1-E3, E4, E6). For independent trainees, voice training resources like Sumian Voice \cite{sumian_voice_examples} provide a (small but growing) database of voices alongside rough character and parameter descriptions which can guide approximate goals to clear goals (E1, E5). E2 likened the experience of finding a clear goal to putting together an outfit:
\begin{quote}
\textit{``I use this analogy of going to a clothing store and trying on different pieces of an outfit and piercing it together. So we're trying on different resonance qualities. We're trying on different pitch centers, different articulation styles... And then kind of piercing together their goal voice.''}
%Extra sections if I have time: "Goals are not targets!" and "Multiple Goals"
\end{quote}
\subsection{Characteristics of Goal Exploration.}
\label{sec:findings:characteristics_of_voice_exploration}
While trainees usually begin with approximate goals when starting voice training, the exact direction provided by clear goals allows for more exact voice practice (E1-E3). We define \textit{goal exploration} as the process through which trainees and experts arrive at clear goals. We found that effective goal exploration accounted for the dynamic nature of goals through continuous reevaluation and benefited from voice models as examples who could demonstrate a range of voices. Furthermore, we identified rigid goals as barriers to the voice training journey and de-emphasis of the goal as a necessary step during troughs and plateaus of progress associated with skill-building and voice generalization.

\subsubsection{Goals Change.}
While a major focus of goal voice exploration is finding a voice ``end''-goal, voice training goals are hardly ever static. Instead, they dynamically evolve as trainees build new skills, discover new aspects of their identity, and perceive the changing qualities of their voices. Experts and trainees continue reevaluating goals throughout the voice training journey to maintain a goal that represents the trainees' voice needs.

\textbf{\textit{Why Goals Change.}} The suitability of a goal depends on both factors inherent to voice training (e.g. motivation, skill, knowledge, and voice physiology) (T3-T5, T7, T9, and all experts) and other personal factors (e.g. identity and environment). As trainees develop their skills and knowledge, their understanding of what is achievable expands (E4, E5, E6). This awareness leads to a recalibration of goals, as trainees pursue more ambitious or nuanced voice characteristics. The effort a trainee invests in voice training is linked to their motivation, which changes throughout the training journey (T4, T8, T9 and E2, E6). Progress often serves as a powerful motivator, encouraging trainees to set more challenging goals (T9). Conversely, periods of perceived stagnation may lead to a reevaluation of goals, resulting in more realistic or achievable goals (T9, T10 and E1, E2). As trainees develop their identity, trainees shift their goals to align with their evolving sense of self (T1, T4, T7, T10). Changes in a trainee's environment (e.g. work or living situation) can necessitate adjustments to voice goals or require trainees to maintain multiple context-dependent goals (T1, T2, T5-T10 and E1, E2, E5, E6).

\textbf{\textit{Continuous Reevaluation.}} Voice experts emphasized the importance of reevaluating client satisfaction and well-being throughout the goal-setting and training process. Rather than imposing specific targets, most of the experts (all but E4) emphasized the need to check in regularly on clients' personal comfort and satisfaction with their voices. All experts mentioned that they regularly employed subjective satisfaction-measurement techniques, such as surveys at the beginning of each session. This technique not only gave clients agency in exploration of voice goals, but also allowed for dynamic goal-setting that accommodated for skill and knowledge development among clients (E6), increasing range with exercising the vocal muscles (E1, E2, E6), and other factors that changed clients' goals, such as changes in overall transition goals (E2, E5, E6).
% \begin{quote}
% ``I work together with them to set a target and a lot of times it's an evolving target. Instead of saying well we are here and I want your endpoint to be here, we talk more about characteristics of voices.'' (P2\_expert)
% \end{quote}
%TODO: new quote from expert here
This approach allows for flexibility in goal-setting and acknowledges the individual nature of voice goals. Trainees (T1-T4) also recognized the importance of personal satisfaction with the goal as other factors changed through the voice training journey, often adjusting their goals as they progressed. For T2 and T10, the impacts of testosterone allowed them to focus less on goals, instead appreciating the progress and forming their voices around the natural changes. T1 shared that their voice goals changed with their personal relationship with voice:
\begin{quote}
``[M]aybe that was an achievable goal, but it wasn't really what I wanted anymore. And my goals sort of shifted to having more acceptance with my voice, whatever that means in any form.''
\end{quote}

\subsubsection{What Makes a Good Voice Example?} We asked trainees and experts about the types of examples that they used as part of the goal exploration process. For trainees who had examples playing a key role in their goal exploration, the best voice models were people who had a set of voices and flexible range, rather than a single voice, as these models demonstrated the ability to change voice. For voice experts, using examples that demonstrated the full variability of voice allowed them to deconstruct clients' negative perceptions about their voices and shift understanding to the voice as a moldable ``instrument'' (E3, E5, E6). Examples grounded in the trainee's identity, such as other trans people and examples produced through modifications of the trainee's voice, provided clarity to the voice training journey. Furthermore, both trainees and experts recognized the power of centering voice exploration around activities where mimicry is already accepted, such as voice acting or singing.

%Voice actors
\textbf{\textit{Voice Actors.}} Voice actors, who could produce a diverse set of voices from a single vocal ``instrument'', aided trainees in understanding the flexibility of voice (T5, T10 and E6). For T5, the ability of voice actors to produce new voices through minor alterations in various vocal parameters (e.g. pitch, resonance, fry) provided her with a starting point for understanding how these parameters could impact her voice. Experts found that using the framing of voice acting characters, such as in role-playing environments like DnD, afforded trainees more comfort in trying out new voices (E1, E5, E6). E6 found that briefly ``trying on'' voices in-session through approximating the voices of various characters from media helped trainees develop direction to a voice goal.
%Singing
%Singing-training and gender-affirming voice training methodologies are interconnected, as both involve increasing vocal ranges and building skill in managing the fluctuation of vocal characteristics through methods such as vibrato or intonation.

\textbf{\textit{Singers.}} Three trainees found that among voice examples, singers were the most effective for their goal voice exploration (T2, T9, T10). Singing provided a route for trying out voices that didn't have the same baggage as mimicking other voice examples (T9, T10). For T2, mariachi singers provided culturally relevant examples of voices that he could mimic, since he didn't hang around too many Spanish-speaking friends. For T9, the range and flexibility of singing helped her find voice examples in her accessible range, allowing her to immediately use them for training and break through the psychological barriers preventing her from training, \textit{``My goal for the first several months was just to not be miserable with it, and so, [for] most of the earlier training, [I] was just singing in the shower.''}

\textbf{\textit{Other Trans People.}} For trainees with unclear journeys to their goal voice, examples of how transgender people changed their voices, such as those available through voice training media like TransVoiceLessons on YouTube \cite{transvoicelessons_youtube} and the trans community around them, demonstrated the timeframe that they could expect for voice training, while also giving them an idea of what their voice would sound like throughout the journey (T2, T5). Given trainees' difficulty in estimating the length of the voice journey (T3, T5, T7-T10), with many trainees feeling reaching a goal voice was impossible (T1-T3, T5, T8-T10), these examples of successful voice training allowed trainees to more aggressively set their end-goals (T5).

\textbf{\textit{My(modified)self.}} While not always providing natural-sounding voices, basic voice changer technologies --- such as voice filters, desktop applications, and advanced vocal processors --- provided inspiration for voice training through examples grounded in trainees' own voices (T1, T3, T4, T6, T7, T9, T10). We found that the impact of voice changer technologies on goal exploration varied with the effectiveness of the software in producing a natural-sounding voice and the technical knowledge of trainees in navigating difficult interfaces for producing a voice. For trainees with imperfect experiences with voice changers, the produced voice could still provide a direction to work towards (T1, T4, T8), and an understanding of the limitations of shifting single characteristics of voice (T9), or specific characteristics to assimilate into their own voices (T1, T6). When voice changers provided adequate voices that allowed trainees to present their identities, trainees felt that the voice changer voice unearthed their own potential, as it demonstrated what voice training could do for them (T1, T10). For T1, positive reactions from others to the modified voice increased internalization, functioning as a motivation for voice training:
\begin{quote}
    \textit{``I did produce something that I think was a very passable cis woman's voice. And I remember sharing that with people and them being like, `I can't believe that was you'... I think I really internalized that people are responding with the sort of shock or disbelief that that could even have been me. And that's the response I want.''}
\end{quote}
\subsubsection{Rigidity Around Goals Stalls Voice Training}
While clear goals provide direction to voice training, rigidity around voice goals serves as a potential barrier, especially during the early skill-building and later voice generalization phases of voice training. To combat goal rigidity, experts reduce focus on the voice goal and emphasize incremental targets and progress.

\textbf{\textit{Rigidity Around Unsustainable Goals.}} Experts noted that trainees were often set on unsustainable or unsuitable voice goals, especially early in the voice training journey (E1-E3, E5, E6). These unsustainable goals resulted in trainees straining their voices through unhealthy practice (T1, T5, T7, T10 and E1, E3, E5) while also demoralizing trainees because of the distance to the goals (T8, T9 and E3). While experts worked with clients to help them understand voice limitations in relation to the goal (E2, E3, E5), this practice could demotivate trainees while also not representing the plasticity of voice. As an alternative strategy, experts temporarily de-emphasize the goal voice while focusing on incremental targets (E1, E2). E2 mentioned how they use this technique:
\begin{quote}
    \textit{``I feel like it can start a shame spiral with some people, like `I'm so far away from this goal voice or this person's voice that I was listening to' ... I think in the beginning we might establish, OK, here's where you're starting, [here's where your] fundamental frequency is, and here's where this person that you were listening to is speaking.''}
\end{quote}
 %Include quote here from an expert

\textbf{\textit{The Perfectionist ``Plateau''.}} Voice experts and trainees identified a ``plateau'' to voice training progress following a phase of rapid voice development (T4, T9 and E1, E3). This plateau involved a combination of ``fine-tuning'' work (T4 and E3) and hurdles for voice generalization (E1, E2, E6). As T4 explained, \textit{``Voice training has a really weird learning curve where you start off [and] you don't see a lot of progress and then there's a period where you're like, `oh, I get it now' and then [for] that month you're gonna get a lot of progress and then later on it's a lot of fine-tuning.''} Trainees  struggled with using an imperfect voice-in-training (VIT) outside controlled practice environments when they thought it wouldn't be perfect (T1, T3, T5, T6, T8 and E5, E6). To combat fears around generalization, trainees controlled the contexts where they would use the VIT (T1, T2, T5, T6, T9 and all experts) and all experts recommended starting with practice partners that the trainee felt comfortable with. Furthermore, experts (E1, E4, E5, E6) identified that feedback focused on small achievements could build trainee self-confidence in generalizing their VIT. For example, E5's encouragement focused on specific voice characteristics, \textit{``[G]iving that encouragement that things are sounding good, or you're doing XY and Z well ... [is] setting people up for success knowing that sometimes things are not going to be perfect and that's OK.''}

%TODO: This section actually builds into setting targets -- return to it if I have time to include targets (and if it doesn't impact the scope too much)
% \subsubsection{Identifying Specific Needs}
% Trainees come from a variety of backgrounds, which not only inform the voice goal itself, but also the techniques for goal voice exploration. Trainees and experts identified how various aspects about the trainee and their environment influenced the goal exploration and target-setting process.

% \textbf{\textit{``Toolbox'' of voices}}
% %Focus on trainees

% \textbf{\textit{Accommodating Various Abilities.}} 
% %Focus on experts

% \textbf{\textit{Leveraging Existing Skills.}}
%Focus on trainees and experts


% ``Yeah, sometimes there might be really good examples of like, I really like looking at like voice actors, for example, who might do a lot of different things and show different parameters of their voice.'' (P7\_trainee)
% \end{quote}
%\textbf{\textit{What the example should do}} 
% \textbf{\textit{Examples for Direction}} Given the distance of examples from trainees' current voices at the start of voice training, several experts () recommended against using an example voice as a target for emulation. E3 described her usage of examples as direction-focused, rather than mimicry-focused:
% \begin{quote}
% ``I tend to have the patient talk about what aspects of that person's voice they like or what things that they are trying to work towards instead of trying to emulate that voice in particular.'' (P4\_expert)
% \end{quote}
%\paragraph{Passing as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention of the "diet culture" and "standard of beauty for voice training and how this influences goals around passing
%Mention of how passing is a social-feedback-based goal, and still exists when a clear goal is set, as it functions as a reliable indicator for some trans individuals of 1) whether they are hitting their targets and 2) whether a clear voice goal is sufficient
%\paragraph{Identity representation as a goal}
%Mention trainees and experts who mentioned this as a goal
%How this is as opposed to passing -- represents both gender-conforming and nonconforming identities, while representing other qualities of identity as well, such as culture
%How this guides into clear goals, such as finding examples that match one's identity (culture, accent, age, gender)
%\paragraph{Overcoming voice dysphoria as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention how voice dysphoria can be both a driving factor and barrier to trainees pursuing voice training
%Mention how trainees and experts use comfort with a voice as a factor when transforming the vague goal of overcoming voice dysphoria to clear evaluations of examples for voice goals
%\paragraph{Changing pitch as a goal}
%Mention of how trainees regularly start with vague ideas of what voice training is and the qualities of voice -- from both the experiences of experts with clients and trainees' perspectives
%Mention how voice training technologies, such as pitch-grabbers like voice tools (with pitch as the guidance factor for being "on-target" with a gender), and basic gender-based voice changers (which change only pitch) misinform trainees on the importance of pitch as a factor to "passing" or sounding like they want to sound -- but also how some trainees found that these tools helped them come to this understanding
%Mention how this builds into clear goals, both through:
%1) Developing a clearer knowledge of the limitations of a pitch and the need to include other parameters like resonance and weight
%2) The single parameter being a possible guiding factor for finding voice examples which capture further aspects of voice
% \subsubsection{Models guiding the goal}
% When discussing goal exploration methodology, both trainees and experts mentioned voice-parameter-driven ( and ) and example-driven ( and ) methods for exploring voice goals, alongside methods that used voice examples for demonstrating voice parameters ( and ). 
% \paragraph{Finding voice examples}
% %mention resources where trainees find models including the internet (e.g. Voice Training Media, Singers, Friends online, Youtubers) and the importance to trainees of finding models that match their voice characteristics
% \paragraph{Expert experiences using models to find goal voice}
% %mention how experts find that clients bring in models for how they want to sound, both prompted and unprompted
% \paragraph{Who to model?}
% %mention the types of models that trainees / experts bring in
% \paragraph{Issues of voice ownership and mimicry}
% %mention that copying a model can make voice feel like an impression for trainees -> low sense of ownership
% \subsubsection{Perspectives on Clear Goals}
% \paragraph{Making the expert's job easier}
% %Various points to go over that various experts mentioned -- makes understanding the parameters and voice exercises easier, makes
% \paragraph{The Pitfall of Rigid Goals}
% %expert perspective -- deadset on rigid goals creates perfectionism and loss of motivation
% %trainee perspective -- setting a goal that is too difficul to reach
% \subsubsection{Examples as goal approximation tools}
% Several trainees and experts ( and ) found that a responsible use of voice examples in goal voice exploration involved treating the models not as goals, but instead as both targets to approximate ( and ) and instruments to pull qualities from ( and ).
% \paragraph{Example approximation for goal discovery}
% \paragraph{Extracting vocal qualities from examples}
% \paragraph{Facilitating a responsible understanding of examples}
% %START OF GVD SECTION
% %NOTE: should "brainstorming" subsections like this be moved to the end of the findings section and included in a separate section? -- in which case would it be fine to include references to previous findings sections?
% \subsubsection{Examples as goal approximation tools}
% Several trainees and experts ( and ) found that a responsible use of voice examples in goal voice exploration involved treating the models not as goals, but instead as both targets to approximate ( and ) and instruments to pull qualities from ( and ).
% \paragraph{Example approximation for goal discovery}
% \paragraph{Extracting vocal qualities from examples}
% \paragraph{Facilitating a responsible understanding of examples}
%START OF GVD SECTION
%NOTE: should "brainstorming" subsections like this be moved to the end of the findings section and included in a separate section? -- in which case would it be fine to include references to previous findings sections?
\subsection{Towards a Goal-Voice-Discovery Tool}
\label{sec:findings:towards_a_goal_voice_discovery_tool}
As part of trainee and expert brainstorming, we asked questions related to software-development of a voiced training tool for discovering voice goals, which we named the Goal-Voice-Discovery (GVD) tool. As part of this tool, we would create a large dataset of voice examples using Retrieval-based Voice Conversion (RVC) technology. Based on the interviews, we identified several factors important to voice trainees and voice experts for the use of examples in goal voice exploration, including a need for a diverse range of examples representing various gender identities, cultural identities, ages, and voice archetypes, a way to create a voice goal that voice trainees can foster ownership over as opposed to an impression of someone else, and a flexible approach to understanding examples that guides approximation instead of rigid perfectionism. To address these factors in the context of the GVD tool, we brainstormed various features alongside voice trainees and experts. 

\subsubsection{Filtering and Arranging a Voice Database.}
Voice trainees and experts emphasized the need for a large database of voice models, including various gender, cultural, and age characteristics (T3, T6, T7, T9, T10 and E3, E4, E5). Our research team recognized the need for methods to search, arrange, and filter through such a large database. Methods for filtering, arranging and searching through the voice database included (1) measurable-parameter based methods and (2) model tagging systems requiring human intervention. 

\textbf{\textit{Parameter-based Methods.}} Among parameter-based methods, three techniques emerged, including allowing trainees to define ranges for various vocal parameters including pitch, resonance, and intonation (T2-T7, T9), using voice-analysis techniques such as pitch range measurement to automatically determine if a set of goals are feasible and suitable for the trainee (T1, T6-T10), and allowing trainees to edit parameters directly using a parameter-based voice changer (not RVC) to see what sounds good, either working from their current voice or a voice example (T1).

\textbf{\textit{Tagging Methods.}} Among human-description-based tagging methods, desired voice features included voice accent, such as a valley girl or midwestern accent (T3, T7, T8, T9 and E5), voice archetypes, such as an authoritative feminine voice or a ``pretty boy'' voice (T10 and E3, E6), features of voice not yet directly measurable by voice-analysis software, including breathiness, brightness, and scratchiness (T6, T7 and E3, E4, E5), and characteristics of the person who the model is based on, including emotional characteristics, age and gender (T8, T10). To manage tagging of a large database while also giving trainees agency to describe voices using characteristics understandable to themselves, E6 recommended crowdsourcing methods for voice-tagging, such as those employed by the voice training website Sumian Voice \cite{sumian_voice_wiki}.

\subsubsection{Creating Grounded and Unique Voices.} While full-conversion voice changers could provide a database of voice models representing various identities, trainees worried that directly using another person's voice as a goal would create a low sense of ownership (T1, T6), result in a non-unique voice (T7), or create a voice that was too difficult to achieve (T1, T2, T8 and E3-E5). To address this, we explored various voice-changer-inspired techniques for creating unique voices.

\textbf{\textit{Merging Models.}} To address the problem of voice ownership and individualized voice goals, trainees came up with two use-cases for RVC-model merging. The first was merging multiple voice models together from the database to create unique voices that didn't exist before (T5). The second was creating a model of the trainee's current voice and merging it with the desired model to maintain voice characteristics, grounding the goal voice with characteristics from the trainees' original voice (T1).

\textbf{\textit{Simple Voice Changers.}} A voice-parameter-based voice changer could serve as an extra layer on top of an RVC-based voice changer to allow for further customization in creating a unique voice (T1, T8). Also, pulling understandable parameters from the RVC-based voice changer model to feed a more basic parameter-based voice changer, then modifying the current voice using these parameters could create an approximation that maintains characteristics of the original voice (T1).

%Maybe work into previous section?
\textbf{\textit{Visualizing the journey to a goal.}}
To emphasize the goal as a direction rather than an impression to be perfected, we worked with experts and trainees to determine methods for visualizing the journey towards the goal voice model. Among important features mentioned by trainees and experts were (1) voice parameter measurements of the model, such as pitch, resonance, and pitch range (T1, T5, T7, T9, T10 and E1, E4, E5, E6), (2) effort, difficulty, and time approximations representing the current voice's distance from the model (T3, T6), and (3) milestone models as ``steps'' to the model (T3). To understand the current voice's distance from the model, we discussed (1) merging models between the trainee's current voice and the model voice with varying weights, reducing the current voice weight for increments closer to the model (T3), (2) using voice models that are not directly the end-goal, but currently emulate-able by the trainee for practice in the direction of the goal model (T5, T8), and presenting the journey in a gamified way, such as milestones and rewards used in language-learning applications like Duolingo (T1, T2, T10 and E6).

==> extra_files/old_versions/findings_2.tex <==
% (GVE = Goal Voice Exploration, IVT = Incremental Voice Targets, VG = Voice Generalization)
% - Key Findings Rough Re-organization:
%   - Individualized and nonlinear nature of voice training
%       - Understanding of the voice training journey as a curve from a difficult start to rapid progress and then a plateau where the focus becomes smaller changes in voice and generalizing voice practice to use throughout trainee's daily lives
%       - How experts and trainees work to sustain motivation through the troughs of voice training progress
%       - How responsible and irresponsible technology use function to motivate or demoralize
%   - Heiarchies of understanding voice, voice perception, and comfort, and how they interact with goal discovery, target-setting, and voice generalization + How trainees / experts use technologies to support progression through these heirarchies, including:
%       - (GVE, IVT) Using Voice Training Media (VTM) to develop initial skills/knowledge to better describe and explore voice goals + find examples of what the voice training journey looks like (at multiple points) in transgender individuals, such as Zee from TransVoiceLessons [reference], and pitch-grabber applications as a stepping stone to understanding the functions of various voice parameters in creating a voice
%       - (IVT, VG) Stepping up the perception ladder from voice analysis software to identifying features from voice recordings to building a sense of self-perception via cueing from others and understanding physical sensation -- and how the use of technologies during the first part supports the development of the final perceptual goals
%       - How experts and trainees work through introducing cognitive load into voice practice as a step towards voice generalization and how they use technologies like controlled conversational environments through computer-mediated-communication (CMC) (e.g. voice calls, simulating ordering from a place, short conversations in practice spaces with other trans individuals) and large-language-model generation of scripts to read aloud as stepping stones in this cognitive heirarchy
%       - How experts and trainees move through trainees' individual comfort heirarchies, expanding voice-in-training (VIT) use from environments that are most comfortable to most stressful for the trainees while balancing the need for authentic practice with trainees' perceptions of safety and comfort -- and the role that simulation of conversations, both low-tech and high-tech (our brainstorming + mentioned by some experts) can play in balancing these factors
%   - (GVE) Understanding goal voice exploration as a process with multiple routes of attack, including:
%       - Approximate goals
%       - Clear Goals (Examples, etc.)
%   - (GVE) Interaction between goal discovery and technology use
%       - Using voice changers to explore goals built on top of the trainee's own voice while testing them in online environments such as video games
%       -(Examples, modelling, and mimicry) Finding both transgender and cisgender individuals that match a trainee's identity online, and using these as examples
%       - Using online resources such as Sumian Voice and their (small) voice examples database to understand how models for a goal voice relate to vocal parameters (and thus gaining a small understanding of the journey) [https://wiki.sumianvoice.com/wiki/pages/voice-examples/]
%   - Interaction between incremental target-setting and technology use
%       - How trainees and experts use voice analysis and recordings to identify specific challenges to target
%   - Interaction between voice generalization and technology
%sections from previous findings to work-in:
%section 5.2 will likely get rebuilt into the "goal voice exploration" subsection, and section 5.3 likely won't require too many major structural changes to serve as one of the final findings sections in the new findings structure. Parts from 5.4 will also get worked into the goal voice exploration and first phase of voice training journey sections, and I'll break parts of 5.5 into the second section of the new findings structure (on overall trajectory of voice training journeys) and the progress-motivation section of the findings.
%FIRST: Start with definitions!

%First section: goal voice exploration
\subsection{Goal-Voice Exploration}
\label{sec:findings:subsec:Goal-Voice_Exploration}
%Second (shorter) section: Idea of 3-phase voice training journey and the barriers that define these phases
\subsection{The Nonlinear Voice Training Journey}
\label{sec:Findings:The_Nonlinear_Voice_Training_Journey}
%Third (longer) section: First phase of voice training journey + how technique + technology interacts with it
\subsection{Exploration and Knowledge-Building}
\label{sec:Findings:Exploration_and_Knowledge-Building}
%Fourth (longer) section: Second phase of voice training journey + how technique + technology interacts with it
\subsection{Rapid_Progression_through_Targets}
\label{sec:Findings:subsec:Rapid Progression through Targets}
%Fifth (longer) section: Third phase of voice training journey + how technique + technology interacts with it
\subsection{Hitting the Plateau}
\label{sec:Findings:Hitting_the_Plateau}
%Sixth (short) section: Progress-Motivation cycles and effective methods for maintaining motivation
\subsection{Progress-Motivation Cycles}
\label{sec:Findings:subsec:Progress-Motivation Cycles}
%Seventh section (medium-long): heirarchies of voice training -- specificity (goals + targets), perceptual (measure to listen to feel), 
\subsection{Hierarchies of Voice Training}
\label{sec:Findings:subsec:Hierarchies of Voice Training}

==> extra_files/old_versions/old_discussion.tex <==
Our findings reveal the complex and nuanced nature of gender-affirming voice training, highlighting the need for personalized, flexible, and technologically-enhanced approaches. In this section, we discuss the implications of our results and propose design guidelines for future voice training technologies, particularly focusing on goal voice discovery, incremental target setting, and simulated environments for voice generalization.

\subsection{Universal Guidelines for Voice Training Technologies}

% This subsection discusses overarching principles that should guide the development of voice training technologies, based on our findings from both experts and trainees.

\subsubsection{Acknowledging Changing Goals}

% This subsubsection emphasizes the dynamic nature of voice goals and the importance of technologies adapting to these changes.

\paragraph{Skillset Informing New Goals}
% Discuss how trainees' growing skills and knowledge influence their voice goals
% Reference: Trainee codebook > voice goals > Changing Voice Goals > Goals Changing as a Result of Skill and knowledge-building
% Quote from trainee about how their goals changed as they learned more about voice training

\paragraph{Limitations Informing New Goals}
% Discuss how trainees adjust their goals based on perceived limitations
% Reference: Expert codebook > Client Goals > Client Factors Contributing to Goal > Client  Physiology
% Quote from expert about helping clients set realistic goals based on their physiology

\paragraph{Comfort Informing New Goals}
% Discuss the importance of comfort in goal-setting
% Reference: Trainee codebook > voice goals > Goals that fit oneself
% Quote from trainee about adjusting their goals to find a voice that feels comfortable and authentic

\paragraph{Feedback Informing New Goals}
% Discuss how various forms of feedback shape trainees' goals
% Reference: Expert codebook > Feedback and Motivation > Feedback > Importance of feedback
% Reference: Trainee codebook > Voice training techniques > Social Influences on Voice Training > Social feedback
% Quote from expert about the role of feedback in goal refinement
% Quote from trainee about how social feedback influenced their voice goals

\paragraph{Biological Changes Informing Changing Goals}
% Discuss how hormonal therapy and vocal muscle development affect goals
% Reference: Trainee codebook > Demographics > Voice training progress/experience > testosterone/hormone
% Quote from trainee about how testosterone affected their voice goals

\paragraph{Non-Linear Training Paths}
% Discuss the various paths trainees take in their voice training journey
% Reference: Expert codebook > Voice Training Challenges > Difficulty making progress or achieving target
% Reference: Trainee codebook > Motivation > Making progress > Voice training is an ongoing process
% Quote from expert about the non-linear nature of voice training progress
% Quote from trainee about their non-linear journey in voice training

\subsubsection{Assume Nothing!}

% This subsubsection emphasizes the importance of avoiding assumptions in voice training technology design.

\paragraph{Individualized Goals}
% Discuss the diverse range of voice goals beyond binary gender expectations
% Reference: Trainee codebook > voice goals > Goal for gender presentation
% Quote from trainee about their unique voice goals that defy binary expectations

\paragraph{Multiple Goals for One Trainee}
% Discuss how trainees often have multiple, context-dependent voice goals
% Reference: Trainee codebook > voice goals > Context-Dependent Goals
% Quote from trainee about having different voice goals for different situations

\paragraph{Subjective Goal Setting}
% Discuss the importance of trainee feelings and satisfaction in goal setting
% Reference: Expert codebook > SLP Strategies > Focusing on Client Well-being
% Quote from expert about centering client satisfaction in goal setting

\paragraph{Individualized Comfort with Voice-in-Training (VIT)}
% Discuss varying levels of comfort with using VIT in different contexts
% Reference: Trainee codebook > IVT Techniques > Social Context and VIT-use
% Quote from trainee about their comfort levels using VIT in different situations

\subsubsection{Parameter Focus}

% This subsubsection discusses the importance of focusing on various voice parameters, not just pitch.

\paragraph{Avoiding Overreliance on Pitch}
% Discuss the limitations of focusing solely on pitch in voice training
% Reference: Expert codebook > SLP Strategies > Skill-building > understanding parameters
% Reference: Trainee codebook > Technologies > Voice Tools/Pitch Grabbers > (Too much) emphasis on pitch
% Quote from expert about the importance of parameters beyond pitch
% Quote from trainee about their experience with overemphasis on pitch

\paragraph{Importance of Resonance}
% Discuss the crucial role of resonance in voice training
% Reference: Expert codebook > IVT Techniques > Exercise Techniques > Focusing on Parameters > Exercise techniques: importance of resonance
% Quote from expert about the importance of resonance in voice training

\paragraph{Measurement of Complex Parameters}
% Discuss the need for technologies that can measure and provide feedback on complex voice parameters
% Reference: Expert codebook > Technology  Practices > In-session
% Reference: Trainee codebook > Need for a better tool
% Quote from expert about the limitations of current voice measurement technologies
% Quote from trainee about their desire for more comprehensive voice feedback

\subsubsection{Health and Sustainability Focus}

% This subsubsection emphasizes the importance of maintaining vocal health throughout the training process.

\paragraph{Avoiding Fatigue and Strain}
% Discuss strategies to prevent vocal strain and fatigue
% Reference: Expert codebook > SLP Strategies > Focusing on Client Well-being > making sure clients' voices are healthy and sustainable
% Quote from expert about strategies to prevent vocal strain

\paragraph{Incorporating Vocal Health Exercises}
% Discuss the importance of including vocal health exercises in training regimens
% Reference: Expert codebook > IVT Techniques > Exercise Techniques > Vocal health
% Quote from expert about specific vocal health exercises they recommend

\paragraph{Developing Trainees as "Mini-Clinicians"}
% Discuss the importance of teaching trainees to monitor their own vocal health
% Reference: Expert codebook > SLP Strategies > helping clients build skills and become mini-clinicians
% Quote from expert about strategies to help clients become more self-aware of their vocal health

\paragraph{Acknowledging Bad Days}
% Discuss the importance of flexibility and self-compassion in voice training
% Reference: Trainee codebook > Voice Training Challenges > Other challenges/barriers
% Quote from trainee about dealing with setbacks or "bad voice days"

\paragraph{Addressing Voice Dysphoria}
% Discuss strategies to help trainees work through voice dysphoria
% Reference: Trainee codebook > Voice Training Challenges > Discomfort with voice
% Quote from trainee about their experience with voice dysphoria and strategies to overcome it

\subsubsection{The Expert Still Matters}

% This subsubsection emphasizes the continued importance of voice experts in the training process.

\paragraph{Identifying Vocal Health Issues}
% Discuss the expert's role in monitoring vocal health
% Reference: Expert codebook > SLP Strategies > Focusing on Client Well-being
% Quote from expert about their role in identifying and addressing vocal health issues

\paragraph{Overcoming Psychological Barriers}
% Discuss the expert's role in helping trainees overcome mental blocks
% Reference: Expert codebook > SLP Strategies > Focusing on Client Well-being > importance of feeling safe during voice training
% Quote from expert about strategies to help clients overcome psychological barriers

\paragraph{Expert as Counselor}
% Discuss the counseling aspect of voice training
% Reference: Expert codebook > SLP Strategies > Focusing on Client Well-being
% Quote from expert about their role as a counselor in the voice training process

\paragraph{Guiding Technology Use}
% Discuss the expert's role in helping trainees use voice training technologies effectively
% Reference: Expert codebook > Technology  Practices > Problems with technologies > importance of responsible technology use (and avoidance of over-reliance)
% Quote from expert about guiding clients in responsible technology use

\paragraph{Accessibility Concerns}
% Discuss the issue of expert care being prohibitively expensive for some trainees
% Reference: Trainee codebook > Voice Training Challenges > Other challenges/barriers > Pain-points: finding accessible (financially) resources for voice training
% Quote from trainee about financial barriers to accessing expert care

\paragraph{Expert Involvement in Tool Design}
% Discuss the importance of involving experts in the design of voice training technologies
% Reference: Expert codebook > Brainstorming
% Quote from expert about their perspective on helpful features for voice training technologies

\subsection{Technology Designs}

% This subsection discusses specific technology designs based on our findings and brainstorming sessions.

\subsubsection{Goal Voice Discovery (GVD)}

% This subsubsection focuses on technologies to aid in goal voice discovery.

\paragraph{Guiding Approximate Goals to Concrete Goals}
% Discuss strategies for helping trainees refine their voice goals
% Reference: Expert codebook > Goal Voice Discovery (GVD) > Arranging/Filtering Voices
% Reference: Trainee codebook > voice goals > Changing Voice Goals
% Quote from expert about strategies to help clients refine their voice goals
% Quote from trainee about their experience refining their voice goals

\paragraph{Voice Conversion and Enhancement Technologies}
% Discuss the potential of AI voice changers and "analog" voice changers in goal voice discovery
% Reference: Expert codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG) > voice changers
% Reference: Trainee codebook > Technologies > Voice changers
% Quote from expert about the potential benefits and risks of voice changer technology
% Quote from trainee about their experience or thoughts on using voice changers for goal exploration

\paragraph{Database Diversity}
% Discuss the importance of a diverse voice model database
% Reference: Expert codebook > Goal Voice Discovery (GVD) > Desired goal voices
% Reference: Trainee codebook > voice goals > Goals focused on mimicry
% Quote from expert about the importance of diverse voice models
% Quote from trainee about their experience finding relatable voice models

\paragraph{Filtering and Arranging Voice Models}
% Discuss strategies for organizing and navigating a large voice model database
% Reference: Expert codebook > Goal Voice Discovery (GVD) > Arranging/Filtering Voices
% Reference: Trainee codebook > Brainstorming > Goal Voice Discovery (GVD) > Arranging/Filtering Voices
% Quote from expert about effective ways to organize voice models
% Quote from trainee about their preferences for exploring voice models

\paragraph{Estimating the Voice Training Journey}
% Discuss methods for providing trainees with realistic expectations of their voice training journey
% Reference: Expert codebook > Client Goals > Voice Training Perceived Timeline
% Reference: Trainee codebook > voice goals > Achievability of goals > Voice Training Perceived Timeline
% Quote from expert about setting realistic expectations for voice training progress
% Quote from trainee about their experience with the voice training timeline

\paragraph{Proposed GVD Model}
% Present a model for a Goal Voice Discovery tool based on our findings
% Reference: Expert codebook > Brainstorming > Goal Voice Discovery (GVD)
% Reference: Trainee codebook > Brainstorming > Goal Voice Discovery (GVD)
% [Include a figure of the proposed GVD model here]
% Describe the key components and workflow of the proposed GVD model

\subsubsection{Voice Exercises Towards Incremental Goals (VETIG)}

% This subsubsection focuses on technologies to aid in setting and achieving incremental voice training goals.

\paragraph{Small Incremental Goals}
% Discuss the importance of setting small, achievable goals
% Reference: Expert codebook > VETIG (Voice Exercises Towards Incremental Goals) > Benefits of Incremental Goals
% Reference: Trainee codebook > IVT Techniques > Target-setting > Setting small and specific targets
% Quote from expert about the benefits of small, incremental goals
% Quote from trainee about their experience with small, incremental goals

\paragraph{Working on Voice Aspects Separately and Combining}
% Discuss strategies for isolating and then combining voice aspects in training
% Reference: Expert codebook > VETIG (Voice Exercises Towards Incremental Goals) > Working on parameters
% Reference: Trainee codebook > voice goals > Factors that influence goals > Focus on Parameters/Techniques
% Quote from expert about strategies for working on individual voice aspects
% Quote from trainee about their experience working on different voice aspects

\paragraph{Parameter Goals vs. Mimicry}
% Discuss the benefits and challenges of parameter-based goals versus mimicry-based goals
% Reference: Expert codebook > Client Goals > Approximate Goals > How Clients Describe Goals
% Reference: Trainee codebook > voice goals > Goals focused on mimicry
% Quote from expert about balancing parameter-based and mimicry-based approaches
% Quote from trainee about their experience with parameter-based vs. mimicry-based goals

\paragraph{Proposed "LEAP" Model}
% Present a model for an incremental voice training tool based on our findings
% Reference: Expert codebook > Brainstorming > VETIG (Voice Exercises Towards Incremental Goals)
% Reference: Trainee codebook > Brainstorming > VETIG (Voice Exercises Towards Incremental Goals)
% [Include a figure of the proposed LEAP model here]
% Describe the key components and workflow of the proposed LEAP model

\subsubsection{Simulated Environments for Voice Generalization (SEVG)}

% This subsubsection focuses on technologies to aid in voice generalization through simulated environments.

\paragraph{Benefits of Simulated Environments}
% Discuss how simulated environments can complement real-world practice
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Practice Environments and Activities
% Reference: Trainee codebook > IVT Techniques > Conversational Targets > Generalizing Voice
% Quote from expert about the benefits of simulated practice environments
% Quote from trainee about their experience or thoughts on simulated practice environments

\paragraph{Managing Safety and Stress with Voice Changers}
% Discuss how voice changers can be used to create safe practice spaces
% Reference: Expert codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG) > VC as an enhancement
% Reference: Trainee codebook > Technologies > Voice changers > Voice changer potential for goal exploration / testing voices
% Quote from expert about using voice changers to create safe practice environments
% Quote from trainee about their experience or thoughts on using voice changers for practice

\paragraph{Enhanced Feedback in Simulated Environments}
% Discuss how simulated environments can provide more detailed feedback
% Reference: Expert codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG) > information to show on HUD
% Reference: Trainee codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG) > information to show on HUD
% Quote from expert about potential enhanced feedback in simulated environments
% Quote from trainee about their desired feedback in practice environments

\paragraph{Proposed SEVG Model}
% Present a model for a Simulated Environment for Voice Generalization tool based on our findings
% Reference: Expert codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG)
% Reference: Trainee codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG)
% [Include a figure of the proposed SEVG model here]
% Describe the key components and workflow of the proposed SEVG model

\subsection{Bridging Expert and Trainee Perspectives}

% This subsection discusses how the proposed technologies can address the gap between expert knowledge and trainee experiences.

\paragraph{Leveraging Expert Knowledge}
% Discuss how the proposed technologies incorporate expert knowledge
% Reference: Expert codebook > SLP Strategies
% Quote from expert about important voice training principles to incorporate into technologies

\paragraph{Addressing Trainee Needs}
% Discuss how the proposed technologies address specific trainee needs and challenges
% Reference: Trainee codebook > Voice Training Challenges
% Quote from trainee about specific challenges they face in voice training

\paragraph{Promoting Responsible Technology Use}
% Discuss strategies for ensuring responsible use of voice training technologies
% Reference: Expert codebook > Technology  Practices > Problems with technologies > importance of responsible technology use (and avoidance of over-reliance)
% Reference: Trainee codebook > Technologies > Voice Tools/Pitch Grabbers > Pitch Grabber / Voice Tools as stepping stone to self-monitoring / perception
% Quote from expert about guidelines for responsible technology use
% Quote from trainee about their experience learning to use voice training technologies responsibly

\subsection{Limitations and Future Work}

% This subsection discusses the limitations of the current study and potential directions for future research.

\paragraph{Study Limitations}
% Discuss limitations such as sample size, qualitative nature of the study, etc.
% [No specific references needed, as this is a reflection on the study itself]

\paragraph{Future Technology Development}
% Discuss potential next steps in developing and evaluating the proposed technologies
% Reference: Expert codebook > Brainstorming
% Reference: Trainee codebook > Brainstorming
%%

==> extra_files/old_versions/old_findings.tex <==
Our findings reveal the complex and individualized nature of gender-affirming voice training, highlighting the importance of trainee-driven goal exploration, hierarchical approaches to training, and the need for flexible, context-dependent goals. We also uncover the challenges trainees face and the strategies that trainees and experts employ to help trainees stay motivated and generalize their newly acquired voice skills.
%TODO: This section needs to be reframed in some way or combined into another
\subsection{Trainee-Driven Goal Exploration}

Our interviews with experts and trainees reveal that the process of discovering and refining voice goals is predominantly trainee-driven, with voice experts and online voice training resources playing a supportive role in guiding this exploration. This section explores the various aspects of goal exploration, from the initial stages of goal setting to the development of a sense of ownership over the voice.

\subsubsection{Voice Experts Centering Clients on Subjective Satisfaction}

Voice experts emphasize the importance of client satisfaction and well-being throughout the goal-setting and training process. Rather than imposing specific targets, many of the experts (all but P5E) emphasized the need to focus on clients' personal comfort and satisfaction with their voices. Multiple experts (P?E, P?E, P?E) mentioned that they regularly employed subjective satisfaction-measurement techniques, such as surveys at the beginning of each session. This technique not only gave clients agency in exploration of voice goals, but also allowed for dynamic goal-setting that accommodated for skill and knowledge development among clients (), increasing range with exercising the vocal muscles (), and other factors that changed clients' goals, such as changes in overall transition goals. As P?E explained:

% \begin{quote}
% ``I work together with them to set a target and a lot of times it's an evolving target. Instead of saying well we are here and I want your endpoint to be here, we talk more about characteristics of voices.'' (P2\_expert)
% \end{quote}
%TODO: new quote from expert here

This approach allows for flexibility in goal-setting and acknowledges the individual nature of voice goals. Several trainees () also recognized the importance of personal satisfaction, often adjusting their goals as they progressed. P3T shared that their voice goals changed with their personal relationship with voice:
\begin{quote}
``And that definitely changed over time where I felt like, yeah, maybe that was an achievable goal, but it wasn't really what I wanted anymore. And my goals sort of shifted to having more acceptance with my voice, whatever that means in any form.'' (P3\_trainee)
\end{quote}
%TODO: work this in here or somewhere else
\begin{quote}
``I would say the majority of the time it's a lot of like self exploration. I use this analogy of going to a clothing store and like trying on different pieces of an outfit and like piercing it together. So we're trying on different like resonance qualities. We're trying on different pitch centers, different articulation styles... And then kind of piercing together their goal voice.'' (P3\_expert)
\end{quote}
% \subsubsection{Finding Voice Models for Goal Voice Exploration}

% Both trainees and experts utilize voice examples to aid in goal setting and exploration. Trainees often seek out inspiring voices to emulate or draw characteristics from:

% \begin{quote}
% ``Yeah, sometimes there might be really good examples of like, I really like looking at like voice actors, for example, who might do a lot of different things and show different parameters of their voice.'' (P7\_trainee)
% \end{quote}

% Experts support this process by helping clients identify specific qualities they appreciate in model voices:

% \begin{quote}
% ``Don't routinely. I've had a handful of patients that come in with celebrities or, you know, famous people in mind, and we will typically listen to that person's voice together. But instead of kind of the mimicking piece, I tend to have them, the patient talk about what aspects of that person's voice they like or what things that they are trying to work towards instead of trying to emulate that voice in particular.'' (P4\_expert)
% \end{quote}

%Strategy for this section: mentions of technology whithin discussion of the voice-training-related finding, building into section from the brainstorming section bringing everything together into a technical finding
%NOTE: this section is on-track, but might be too large + need some way to build in the goal voice exploration activities -- maybe split approximate and clear goals into separate sections?
\subsection{Balancing the benefits of clear goals with the downsides of rigid goals}
When discussing goal voice exploration techniques with experts and trainees, two types of goals emerged: approximate goals, where the trainee knows some details about the direction that they'd like to take their voice, and clear goals, where the trainee has an exact voice area that they're aiming for. Trainees defined approximate goals in terms of:
\begin{itemize}
    \item Utility of the voice, such as having a voice that passes
    \item Representation of their identity, such as having a voice that better represents their gender
    \item A need for personal satisfaction with the voice, such as a voice that doesn't cause dysphoria, or
    \item Basic single-parameter explanations, such as wanting a higher or lower pitch
\end{itemize}
 Trainees defined clear goals in terms of:
 \begin{itemize}
     \item Archetypes, such as ``someone who could rock a ball gown but then get in a fight in a bodega'' or ``pretty boy''
     \item Clear combinations of voice parameters, such as fry, weight, resonance, and pitch, or
     \item Examples of voices that the trainee wanted to sound like, both from around them and through online resources and media
 \end{itemize}
While clear goals allowed for more directed practice for trainees and therapy methods for experts when compared to approximate goals, clear goals also posed a risk of becoming rigid targets, enforcing perfectionism.
\subsubsection{Approximate Goals}
When in the initial stages of voice training or when originally seeing a voice expert, some trainees have vague ideas of what they want out of their voices, but lack the language, knowledge, skills, or examples to define a clear voice goal. Specific examples of these approximate goals mentioned by trainees and experts included passing as cisgender, representing their gender-conforming or nonconforming identity, overcoming gender dysphoria around voice, or changing a single parameter of voice, such as pitch. While these approximate goals make way to clearer goals as voice training progresses, they still impact how trainees and experts set and evaluate clear goals.
\paragraph{Passing as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention of the "diet culture" and "standard of beauty for voice training and how this influences goals around passing
%Mention of how passing is a social-feedback-based goal, and still exists when a clear goal is set, as it functions as a reliable indicator for some trans individuals of 1) whether they are hitting their targets and 2) whether a clear voice goal is sufficient
\paragraph{Identity representation as a goal}
%Mention trainees and experts who mentioned this as a goal
%How this is as opposed to passing -- represents both gender-conforming and nonconforming identities, while representing other qualities of identity as well, such as culture
%How this guides into clear goals, such as finding examples that match one's identity (culture, accent, age, gender)
\paragraph{Overcoming voice dysphoria as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention how voice dysphoria can be both a driving factor and barrier to trainees pursuing voice training
%Mention how trainees and experts use comfort with a voice as a factor when transforming the vague goal of overcoming voice dysphoria to clear evaluations of examples for voice goals
\paragraph{Changing pitch as a goal}
%Mention of how trainees regularly start with vague ideas of what voice training is and the qualities of voice -- from both the experiences of experts with clients and trainees' perspectives
%Mention how voice training technologies, such as pitch-grabbers like voice tools (with pitch as the guidance factor for being "on-target" with a gender), and basic gender-based voice changers (which change only pitch) misinform trainees on the importance of pitch as a factor to "passing" or sounding like they want to sound -- but also how some trainees found that these tools helped them come to this understanding
%Mention how this builds into clear goals, both through:
%1) Developing a clearer knowledge of the limitations of a pitch and the need to include other parameters like resonance and weight
%2) The single parameter being a possible guiding factor for finding voice examples which capture further aspects of voice

\subsubsection{Models guiding the goal}
When discussing goal exploration methodology, both trainees and experts mentioned voice-parameter-driven ( and ) and example-driven ( and ) methods for exploring voice goals, alongside methods that used voice examples for demonstrating voice parameters ( and ). 
\paragraph{Finding voice examples}
%mention resources where trainees find models including the internet (e.g. Voice Training Media, Singers, Friends online, Youtubers) and the importance to trainees of finding models that match their voice characteristics
\paragraph{Expert experiences using models to find goal voice}
%mention how experts find that clients bring in models for how they want to sound, both prompted and unprompted
\paragraph{Who to model?}
%mention the types of models that trainees / experts bring in
\paragraph{Issues of voice ownership and mimicry}
%mention that copying a model can make voice feel like an impression for trainees -> low sense of ownership
\subsubsection{Perspectives on Clear Goals}

\paragraph{Making the expert's job easier}
%Various points to go over that various experts mentioned -- makes understanding the parameters and voice exercises easier, makes
\paragraph{The Pitfall of Rigid Goals}
%expert perspective -- deadset on rigid goals creates perfectionism and loss of motivation
%trainee perspective -- setting a goal that is too difficul to reach
\subsubsection{Examples as goal approximation tools}
Several trainees and experts ( and ) found that a responsible use of voice examples in goal voice exploration involved treating the models not as goals, but instead as both targets to approximate ( and ) and instruments to pull qualities from ( and ).
\paragraph{Example approximation for goal discovery}
\paragraph{Extracting vocal qualities from examples}
\paragraph{Facilitating a responsible understanding of examples}
%START OF GVD SECTION
%NOTE: should "brainstorming" subsections like this be moved to the end of the findings section and included in a separate section? -- in which case would it be fine to include references to previous findings sections?
\subsubsection{Examples as a piece to a Goal-Voice-Discovery tool}
As part of trainee and expert brainstorming, we asked questions related to software-development of a voiced training tool for discovering voice goals, which we named the Goal-Voice-Discovery (GVD) tool. As part of this tool, we would create a large dataset of voice examples using Retrieval-based Voice Conversion (RVC) technology. Based on the interviews, we identified several factors important to voice trainees and voice experts for the use of examples in goal voice exploration, including a need for a diverse range of examples representing various gender identities, cultural identities, ages, and voice archetypes, a way to create a voice goal that voice trainees can foster ownership over as opposed to an impression of someone else, and a flexible approach to understanding examples that guides approximation instead of rigid perfectionism To address these factors in the context of the GVD tool, we brainstormed various features alongside voice trainees and experts. 

Voice trainees and experts emphasized the need for a large database of voice models, including various gender, cultural, and age characteristics. Our research team recognized the need for methods to search, arrange, and filter through such a large database. Methods for filtering, arranging and searching through the voice database included 1) measurable-parameter based methods and 2) model tagging systems requiring human intervention. Among parameter-based methods, several techniques emerged, including allowing trainees to define ranges for various vocal parameters including pitch, resonance, and intonation (), using voice-analysis techniques such as pitch range measurement to automatically determine a set of goals feasible and suitable for the trainee (), and allowing trainees to edit parameters directly using a parameter-based voice changer (not RVC) to see what sounds good, either based on their current voice or a voice example ()

Among human-description-based tagging methods, desired voice features included voice accent, such as a valley girl or midwestern accent (), voice archetypes, such as an authoritative feminine voice or a ``pretty boy'' voice (), features of voice not yet directly measurable by voice-analysis software, including breathiness (), vocal weight (), and scratchiness (), and characteristics of the person who the model is based on, including age and gender (). To manage tagging of a large database while also giving trainees agency to describe voices using characteristics understandable to themselves, P7E recommended crowdsourcing methods for voice-tagging, such as those employed by the voice training website Sumian voice \ref{sumian_voice}.

Several trainees () desired an individualized voice unique to them that mimicry of another person could not provide. As methods for creating goals that trainees could foster a sense of ownership over, we discussed the possibility of merging voice models. In brainstorming the use of this technology as it applies to the problem of voice ownership and individualized voice goals, two use-cases emerged for RVC-model merging, including merging multiple voice models together from the database to create new voices that didn't exist before () and creating a model of the trainee's current voice and merging it with the desired model to maintain voice characteristics ().

We also discussed the use of more basic parameter-based voice changers, with integrations into the GVD system including voice-parameter-based voice changers instead of full-conversion on the trainee's original voice to maximize likeness to the original voice at the cost of the goal model not necessarily sounding natural (). These included using voice-parameter-based voice changers as an extra layer on top of an RVC-based voice changer to allow for further customization in creating a unique voice (), and pulling understandable parameters from the RVC-based voice changer model to feed a more basic parameter-based voice changer, then modifying the current voice using these parameters to create an approximation that maintains characteristics of the original voice ().
%
\paragraph{Visualizing the journey to a goal}
To emphasize the goal as a direction rather than an impression to be perfected, we worked with experts and trainees to determine methods for visualizing the journey towards the goal. Among important features mentioned by trainees and experts were:
\begin{itemize}
    \item Voice parameter measurements of the model, such as pitch, resonance, and pitch range ( and ) to understand the current voice's distance from the model
    \item Merged models between the trainee's current voice and the model voice with varying weights, reducing the current voice weight for increments closer to the model ()
    \item Providing voice models that are not directly the end-goal, but currently emulate-able by the trainee for practice in the direction of the goal model ()
    \item Returning to GVD at various points in the voice training journey to re-evaluate goals based on new understandings of voice limitations and flexibility ()
\end{itemize}
%END OF GVD SECTION
% \subsubsection{Trying Voices to Determine Goals}

% Voice approximation and experimentation play a crucial role in goal discovery. Experts encourage clients to explore different voice qualities:

% \begin{quote}
% ``I would say the majority of the time it's a lot of like self exploration. I use this analogy of like going to a clothing store and like trying on different pieces of an outfit and like piecing it together. So we're trying on different like resonance qualities. We're trying on different pitch centers, different articulation styles.'' (P3\_expert)
% \end{quote}

% Trainees often engage in extensive voice experimentation to find their desired sound:

% \begin{quote}
% ``Yeah. So definitely like voice acting, right? I was. So there are like voice trials on voice actor, voice actor website. Not that I was trying for it, but I just like would read the summary and then try to. I would record myself and try to engage and what I feel that character would convey.'' (P12\_trainee)
% \end{quote}

% \subsubsection{Mimicry and the Feeling of Voice as an Impression}

% The process of mimicry can sometimes lead to a lowered sense of ownership over the voice, especially in the early stages of training. Some trainees report feeling like they're doing an impression rather than speaking in their own voice:

% \begin{quote}
% ``I'm trying too hard, or it's sort of distracting in some way.'' (P3\_trainee)
% \end{quote}

% This sentiment highlights the challenge of integrating new voice qualities while maintaining a sense of authenticity.

% \subsubsection{Gaining Ownership Over a Goal Requires a Clear Path}

% Trainees' perception of effort, difficulty, and distance from their goal significantly affects their sense of ownership over their voice. As trainees gain a better understanding of the path to their goal, their sense of ownership often increases:

% \begin{quote}
% ``When I initially started, it didn't even necessarily feel totally possible. I guess so, like my my goal voice was not something that I even felt like I could fully reach. Whereas at this point I feel like it is reachable, I feel like it's within sight, it's just a matter of getting there.'' (P7\_trainee)
% \end{quote}

% This shift in perception can be crucial for maintaining motivation and progress in voice training.

% \subsubsection{Clients Using Voice Recordings and Direct Feedback for Personal Satisfaction}

% Self-feedback through recordings and real-time audio feedback plays a significant role in trainees' assessment of their progress and satisfaction with their voice:

% \begin{quote}
% ``Yes, I do that a lot. That's actually one of my main methods of of, like measuring my progress.'' (P12\_trainee)
% \end{quote}

% However, some trainees find listening to recordings challenging, especially in the early stages of training:

% \begin{quote}
% ``I could not record my voice is because it was like I could tell how far away I was all the time. And yet I still had to have some fun with singing.'' (P11\_trainee)
% \end{quote}

% Experts often encourage the use of recordings as a tool for self-assessment and tracking progress over time:

% \begin{quote}
% ``I use it for visual feedback so. For example, well, I'll use voice tools if we are finding pitch, so we'll, you know, go from what? Their current speaking fundamental frequency is and then go up and I'll I use humming a lot and hum to where they could still feel comfortable resonance and then we we'll try some words and phrases.'' (P2\_expert)
% \end{quote}
%NOTE: on-track, but wide in scope -- overlaps with other sections
\subsection{Hierarchies in Voice Training and Therapy}

Voice trainees and experts revealed that successful voice training often follows hierarchical patterns, allowing trainees to build skills progressively and tackle challenges in small, achievable pieces. These hierarchies span various aspects of voice training, from target specificity to perceptual skills, cognitive demands, practice environments, and health considerations. Trainees and experts identified technologies allowing trainees to best tackle voice training challenges in a hierarchical method, including:
\begin{itemize}
    \item Voice analysis and recording technologies for identifying specific parts of speech and voice qualities to focus on when setting incremental targets
    \item Voice analysis and recording technologies for building independence in self-perception of voice
    \item Reminder and calendar applications for creating and sustaining vocal habits for making the voice-in-training (VIT) natural
    \item Safe and supportive online social groups as a low-stress environment for using the voice-in-training before moving onto more stressful environments
\end{itemize}

\subsubsection{Target Specificity and Spread}
Both voice experts and trainees emphasize the importance of starting with specific, focused targets before expanding to broader speech elements. This approach allows for manageable goals and steady progress, reducing frustration and strain. Voice analysis and recording technologies aid trainees in accurately setting these specific incremental targets.

\paragraph{Specific targets enabling rapid initial progress}

%trainee using specific targets to make rapid initial progress -- getting to the feminine "part"
%P4 expert using very specific targets first -- 'M' and 'N' sounds
\begin{quote}
``So resonance is what I tend to talk about first. That is a lot of exercises focusing on M\&N sounds, in particular those sounds are really easy to feel kind of in the nose and in the face and it kind of helps to bring home that concept of oral resonance or like mouth resonance. Like get the sound out of your throat, bring it up kind of into your mouth.'' (P4\_expert)
\end{quote}

\paragraph{Spreading rapid progress to speech}

%trainee mention on spreading targets to speech

%expert mention on spreading targets to speech -- find another quote here
\begin{quote}
"Then we start to branch out. Obviously, to like functional phrases. Regular sentences with not just M sounds." (P4\_expert)
\end{quote}
\paragraph{Problem identification via recordings and voice analysis}
One trainee described their approach to target specificity:
\begin{quote}
"I see. So I guess I would take that voice thing and then just speak a sentence and then I would record that and listen back to it. And I would like pick out all the consonants I can tell. This is like I picking out all of the the phonemes, consonants and vowels that like have a resonance drop from that baseline, and then I would take those specific consonants and vowels and like train that one one at a time." (P11\_trainee)
\end{quote}
This granular approach allows trainees to focus on specific aspects of their voice, making the training process more manageable and less overwhelming. Experts often guide clients through a similar progression. As one expert explains:
%Expert quote here

\subsubsection{Perceptual Hierarchies}

A key aspect of voice training involves developing perceptual skills, progressing from reliance on technology to independent self-perception. This hierarchy often begins with the use of voice measurement technologies, moves to voice recordings, and ultimately leads to self-perception without external aids.

\paragraph{Pitch grabbers build an understanding of voice parameters}
Many trainees start by using pitch grabber applications to understand and perceive their voice. One trainee shared:

\begin{quote}
"Like you can see in real time how your pitch is hitting and so I can see how I was using my voice and how it would go up. And I was like, well, I kind of wanted to maintain it in the lower range." (P12\_trainee)
\end{quote}
These tools provide immediate feedback and help trainees develop an initial understanding of their voice. However, experts caution against over-reliance on such technologies (). P6E 

%TODO: Fix this quote -- expand it
\begin{quote}
"I try not to be over reliant on it. And I also try not to make other people over reliant on it because I think one of the main things about voices is that they change pitch." (P6\_expert)
\end{quote}
%TODO: connect more to the analysis, might need to be more expert-driven of a finding
As trainees progress, they often move to using voice recordings for self-evaluation. This method allows for more nuanced perception beyond just pitch. A trainee described this process:

\begin{quote}
"I would record myself singing and play it back to myself. And I would do that for hours every day, working any anywhere between 1:00 to 3:00 hours a day while I was working." (P12\_trainee)
\end{quote}

Several experts () mentioned that while developing independent self-perception of voice was a key to success. From the perspectives of both experts () and trainees (), technologies like voice analyzers and voice recordings provided a scaffolding for developing this perception. P2E encourages using voice analysis and recording technologies as stepping stones to building self-perception:
%TODO: expand this quote backward to find the rest of it
\begin{quote}
"A stepping stone to having that internal sense of where your pitch is. I don't think it like with any technology. And I'll I'll say this as a speech pathologist with kind of all the things I work with, any technology I would say it works best if you can fade it because it's not usually something that you're going to be using all the time." (P2\_expert)
\end{quote}
%%
%split the section here? -- maybe focus in on VIT-use heirarchies here since they build off self-perception
%%
\subsubsection{Cognition Hierarchies (Generalization)}

Voice training also involves a hierarchy of cognitive demands, progressing from simple exercises to more complex, real-world applications. This hierarchy is crucial for generalizing voice skills to everyday life.

One expert outlined this progression:

\begin{quote}
"I do recommend that people again go incrementally, like we start with things that don't have a high cognitive load, reading short sentences, counting, you know, reciting things that people know by heart before going into easy conversations with supportive conversational partners before going into, you know, more stressful presenting, you know, in front of a class or at a conference or something like that." (P2\_expert)
\end{quote}
Trainees often discover this need for incremental progression through experience. P5T's struggle with cognitive load %TODO: get the below sentence integrated up here
\begin{quote}
"In public would be where I would be training my voice. So anytime that like my voice like broke or like I didn't like I wasn't consistent with it. I would notice and I would be super stressed out about it because then I'd be having this conversation with something I'd be like forgetting what they're saying because I'm so focused on how I sound." (P5\_trainee)
\end{quote}
% This experience underscores the importance of balancing structured practice with real-world application, and the need for strategies to manage the cognitive load of voice training in various environments.

\subsubsection{Structure, Space, and Comfort Hierarchies for Using VIT}
Both experts and trainees recognize the importance of gradually expanding the environments in which voice training is practiced. This hierarchy moves from controlled, low-stress situations to more challenging, real-world contexts, taking into account the trainee's comfort level.

\paragraph{Concerns about using VIT}
%Concerns about: 
% having the VIT slip during conversation
% others noticing
%NOTE: Could be moved to trainee-driven approaches to voice training if it doesn't fit here
\paragraph{Perceptions of safety are not universal}
%Trainees have contrasting experiences in what they consider as "safe" environments for voice training:
% - some prefer voice training with strangers, but are afraid of using a new voice with those close to them
Trainees hold contrasting experiences of which environments they find safest to start practice in. For some trainees, interactions with strangers have little consequence, as P3T explains:
\begin{quote}
"I feel like there's a lot of situations where it's like this person is a stranger, that I'm going to have a very short interaction with. But it's also a prime opportunity to practice." (P3\_trainee)
\end{quote}
% - some have fears about using the voice with strangers and in new environments, and would prefer working with specific close friends / practice partners
For other trainees (), people close to them provided the most comfortable environment to start using their VIT in, as {} shows in their experience:
%TODO: include quote here (check relevant subthemes for best quote)
\begin{quote}
    
\end{quote}
Some trainees have specific environments they're worried about using their VIT in, such as their workplace, as explained by P10T:
\begin{quote}
``So first, the goal is out and about in public. To be able to sound the way I want and then at home and then with my with my friends. And then gradually bring that into my workspace. That's my goal, and then gradually I think the the harder part will be when I'm doing the public speaking.'' (P10\_trainee)
\end{quote}
For others, their workplaces can offer a unique opportunity for testing their VIT, with P8T mentioning how their lifeguard job's consistent short interactions allowed them to try out new voices:
\begin{quote}
``So I worked as a lifeguard. And one of the things we did was we would wait up like, stand at the top of the slides and tell people when it was safe to go and so. What I did to kind of test the waters about what felt good to me was because those are people, I just have one interaction with them, and I'm saying a few words I'm saying, like, step up to the slide. Now you can go.'' (P8\_trainee)
\end{quote}

\paragraph{Role-play breaks down barriers}
%technology mentions: Vtuber avatars, vr avatars
%Other things to mention: DnD, voice acting, singing

\paragraph{Authentic exercise is the best exercise}
%Expert techniques such as scripting, bringing in materials from the clients' life, hosting sessions in-environment (such as a coffeeshop)

\subsubsection{Building Hierarchies into Voice Exercise towards Incremental Goals (VETIG)}

\paragraph{}
\paragraph{}
\subsubsection{VIT-use Hierarchies in Simulated Environments for Voice Generalization (SEVG)}
\paragraph{}
\paragraph{}
%Drop this?
% \subsubsection{Health (Emotional and Physical) is Above All}

% Throughout the voice training process, both experts and trainees emphasize the paramount importance of maintaining vocal health and emotional well-being. This consideration overrides all other hierarchies and goals.

% Trainees often encounter issues with fatigue or strain when pushing too hard in their training. One trainee shared their experience:

% \begin{quote}
% "I guess for the first couple of weeks it was like the entire day. My voice got sore eventually, so I stopped doing that and then eventually became about like a couple of hours a day." (P11\_trainee)
% \end{quote}

% Experts are acutely aware of these risks and prioritize vocal health in their approach. One expert emphasized the importance of healthy voice production:

% \begin{quote}
% "First we start with overall healthy voice, so we'll start with breathing. Elimination of any unnecessary muscle tension that they start with and some resonance and semi occluded vocal tract exercises." (P2\_expert)
% \end{quote}

% Another expert highlighted the need to balance progress with vocal health:

% \begin{quote}
% "And then always coming back to making sure that when we're doing it that it feels comfortable and it feels healthy and sometimes we have to go back to some of the breathing and voice exercises to reset." (P2\_expert)
% \end{quote}

% These hierarchical approaches in voice training and therapy provide valuable structure and progression for both experts and trainees. By setting specific targets and gradually expanding them, developing perceptual skills, managing cognitive load, expanding practice environments, and prioritizing health, individuals can work towards their voice goals in a systematic and manageable way. However, it's crucial to remain flexible and adapt these hierarchies to individual needs and learning styles, addressing challenges as they arise to ensure effective and sustainable voice training.

%TODO: Move this section into other sections
\subsection{Individualized Needs in Voice Training}

Both the perspectives of trainees and experts highlighted the importance of recognizing and addressing the diverse and individual needs of voice trainees. This individualization is crucial for effective and meaningful voice training outcomes. We found that trainees' goals, targets, and abilities vary significantly based on their backgrounds, and that voice experts play a critical role in tailoring their approaches to meet these unique needs. We also found that online voice training resources and technologies did not always reflect the full diversity of voice training.

\subsubsection{Diverse Goals Dependent on Individual Background}

Voice training goals are deeply influenced by a trainee's personal, cultural, and linguistic background. This diversity in goals reflects the complex interplay between identity, culture, and voice.
\paragraph{Goals Dependent on Identity}
Experts mentioned how trainee voice goals reflected components of their identities, including personality, linguistic background, and cultural background (). For some trainees, their ideal voice is a reflection of the person they want to transition into, %as P3E explains:
% \begin{quote}
% ``I had one client who I will never forget said that their ideal voice would be someone who could rock a ball gown but then get in a fight in a bodega. It's like a very clear like character of what she wanted to sound like.'' (P3\_expert)
% \end{quote}
Several trainees (P4T, P12T, ...) expressed how their cultural and linguistic backgrounds influenced their voice goals. P4T described the complexity of navigating voice goals across different languages:
\begin{quote}
``[I]t's one thing to transition in one language in one culture, but then [...] in Spanish, [...] I don't have a whole lot of peer friends who I speak Spanish with. So it's slightly different voice goals and different voice expectations, too.'' (P4\_trainee)
\end{quote}

Age was another significant factor in shaping voice goals. Both experts () and trainees () recognized that age-appropriate voices were important. P3T mentioned how the ``industry-standard'' heavily-modulated transfeminine voice did not fit her:
\begin{quote}
``I'm not a young girl, I'm a middle-aged woman and I tend to be a stronger individual, and I tend to have a strong voice and I tend to have leadership abilities and a strong opinion and it just doesn't feel right for me to be out there trying to make my voice into something that's a little too modulated, a little too affected, I suppose.'' (P3\_trainee)
\end{quote}
Several trainees (P3T, P11T, ...) also mentioned how voice training methods from online resources, such as Voice Training Media (VTM), were designed with specific voice goals in mind, creating expectations for how a trans voice should sound and producing practice methods that produced vocal qualities as ``side-effects'' of training. P11T described how she developed a Californian ``valley girl'' accent because of the vowel training methods she learned from YouTube, and how this impacted others' perceptions of her:
\begin{quote}
    ``I have ended up with the Valley girl voice just by the way I trained my vowels. I think it pushed me here. Which is funny because I've never lived in California and people pick up on that. They think I'm from California. That's just a side effect of how specifically [I did] my vowel voice training.''
\end{quote}

\subsubsection{Context-Dependent Goals and the Toolbox Approach}

Our research revealed that many trainees and experts recognize the need for flexibility in voice goals, often conceptualized as a ``toolbox of voices'' for different situations. This approach acknowledges that different contexts may require different vocal presentations.

\paragraph{}
\begin{quote}
``I like having a very modular voice like my voice kind of changes depending on my mood, the situation like what I'm talking about and I like that. I like that freedom, that range, but... Yeah, having a more solid resonance, generally deep voice... With the range to like... You know... Speak differently in different situations.'' (P4\_trainee)
\end{quote}

Experts also supported this flexible approach, recognizing that clients often have different needs in various social contexts:

\begin{quote}
``Absolutely. People definitely want to like basically code mix or code switch, either because they may not be disclosed in certain settings or because they feel affirmed by multiple things and want to be able to have access and so... That kind of approach for me philosophically works really well because I, you know, as a singer by background too, I believe in like the the beauty of like cross training and that an instrument should be able to do a bunch of different things and have the freedom to do a bunch of different things...'' (P7\_expert)
\end{quote}

This toolbox approach extends to bilingual clients as well, with some experts noting that goals for the same client can vary between languages (P5E, ...). P5E noted how trainees wanted different goals between differing linguistic and cultural contexts:
\begin{quote}
``So they may say it's OK if I speak at a lower pitch if I am in Australia, but I really want to speak at a higher pitch if I am in China with my family members.'' (P5\_expert)
\end{quote}

%TODO: build this into other sections
\subsubsection{Tailoring Training Approaches to Individual Needs}

Given the diversity of goals and backgrounds, experts emphasized the importance of tailoring their training approaches to each client's needs. This individualization takes into account not only the client's goals but also their physical capabilities, learning styles, and personal circumstances. One expert described their approach:



Another expert highlighted the importance of working collaboratively with clients to set realistic and achievable goals:

\begin{quote}
``I work together with them to set a target... Instead of saying well we are here and I want your endpoint to be here... I try not to be prescriptive at all. I try to be very... Working together to determine it.'' (P2\_expert)
\end{quote}

\subsubsection{Addressing Diverse Abilities and Challenges}

Our research also revealed that voice training approaches need to account for diverse abilities and challenges faced by trainees. This includes considerations for neurodivergent individuals, as well as those with specific physical or cognitive needs. One trainee with ADHD described their struggle:

\begin{quote}
``I have the ADHD, so it's very hard for me to do like... A sustained effort over time... It's hard to think to have something on your mind... For a long period of time and like I know, that's something that happens with a lot of people who have ADHD. Habit forming is just inherently difficult.'' (P4\_trainee)
\end{quote}

Experts acknowledged these challenges and emphasized the need for tailored strategies:

\begin{quote}
``...we have so many people who are neurodivergent as well. So having like the same response... To touch cues, kinesthetic cues, or visual cues can be a challenge, and then I mostly work through teletherapy, so it's like... It's really about kind of finding the sensory information that is most meaningful.'' (P7\_expert)
\end{quote}


\subsubsection{Leveraging Existing Skills and Experiences}

Finally, our research highlighted how trainees' existing skills and experiences can be leveraged in voice training. Many trainees found that their backgrounds in music, acting, or other voice-related fields provided a valuable foundation for their voice training journey. One trainee explained how their background influenced their perception of voice training difficulty:

\begin{quote}
``Even before I started transitioning, I was always really big into voice acting and so... I have. I have done like, not that I've... Gotten roles, but I have done voice acting... And been pretty proud of my work.'' (P12\_trainee)
\end{quote}

Experts recognized that a client's individual skillset and potential play a significant role in their voice training journey. One expert noted:

\begin{quote}
``Everybody's... Individual skill set is going to be different and potential is different based on like how their system is set up and what their history is like and how much voice work that they've done.'' (P7\_expert)
\end{quote}

Furthermore, experts acknowledged that a client's prior knowledge and experience with voice can significantly influence their goal voice:

\begin{quote}
``A wide variety of kind of initial intake. Some people have come in really depends on a lot of factors, like what part of the kind of like coming out process they're in, and also just like what their level of experiences with voice like. Some people come in with a lot of... A lot of knowledge having maybe come from a singing background and so they have really good idea of what they're looking for'' (P6\_expert)
\end{quote}

These findings emphasize the importance of recognizing and utilizing a trainee's existing skills and experiences in the voice training process. By leveraging these individual strengths and backgrounds, voice training can be tailored to be more effective and meaningful for each trainee.

\subsection{Sustaining Motivation through a  Nonlinear Journey}

Trainees and experts repeated that progress and motivation in voice training are deeply interconnected, forming a cyclical relationship that can either propel trainees forward or hinder their advancement. The nonlinear nature of voice training progress, with an initial lack of clear progress followed by rapid development and a plateau creates many opportunities to both leverage cycles of motivating progress but also creates dips in progress and motivation which can be difficult to overcome. Successful trainees and experts employ techniques such as focusing on incremental progress while avoiding comparisons to the voice goal to maintain motivation throughout the voice training journey.

\subsubsection{Slow, then Rapid, then Plateau}
Voice training is rarely a linear process, as both trainees () and experts () consistently reported. Instead, it often follows a pattern of little progress followed by a breakthrough and rapid progress followed by plateaus, with occasional setbacks. P6T described her experience:
\begin{quote}
``I think training has a very weird learning curve where [when] you start off you don't see a lot of progress. And then there's gonna be a period where you're like, `oh, I get it now' and then [for] that month you're gonna get a lot of progress. And then [when] it's later on it's a lot of fine-tuning and fixing stuff.'' (P6\_trainee)
\end{quote}
This nonlinear progression can be particularly challenging during the initial phases. Experts () noted that clients often struggle with the slow initial development, with P2E noting how the lack of noticeable progress to the endpoint can be frustrating for clients:
\begin{quote}
``There's an intermittent point where the voice isn't where people want it to be, and that's really frustrating because it takes time and so some of it is [...] Sort of learning and starting to know what they need to do, but not having it be at their endpoint yet. I think it's really frustrating.'' (P2\_expert)
\end{quote}
Similarly, trainees echoed this sentiment, with many trainees () describing initial estimates of voice training difficulty as either extremely difficult or impossible (). This perception of difficulty, however, did not necessarily hold, as developing knowledge and a skillset for voice training helped many trainees break out from the initial voice training rut (P4, P5, P7, P11, P12, ...). P4T shared that he broke this perception of voice training through building knowledge from a voice-acting class:
\begin{quote}
    ``[W]hen you're starting to practice, you're like `oh that's impossible.' [...] I had such a high voice [that] it felt impossible until I absolutely needed to do it and I had the space, the support, and the textbooks [...] and once I started it, it became a lot more achievable.''
\end{quote}
% \begin{quote}
% ``I mean, my most rapid progress was in the last two months like [...] Yeah, I I'm not sure here [...] Yeah, my my estimate was not accurate in the sense that like [...] I'm really fast learner so.'' (P11\_trainee)
% \end{quote}
%TODO: find better quote
Experts recognized the motivational impact of this rapid progress phase but also cautioned about the stark contrast of the plateau. P6E mentioned that this plateau often follows as a result of challenges with generalizing voice training progress to conversational settings:
\begin{quote}
``[At] the middle to end, there's often kind of a plateau, right? We get through the easy stuff, it feels comfortable to do the good pitch. We've got a good pitch, sounds good, sounds easy, feels easy [...] We've got that and then we've got a couple resonance things that we can do pretty consistently and like read wrote speech, right. So you can read and have that good resonance and have that good pitch, whatever it is, and that's good. And that's usually a pretty that's a plateau place because [...] After that it's just more difficult.'' (P6\_expert)
\end{quote}
%TODO: transition sentence here
%TODO: include another subsubsection on the negative impacts of perfectionism created by voice analysis tools fuels a cycle of demotivation while making trainees more likely to sucumb to strain and fatigue?
\subsubsection{Focusing on Incremental Progress Sustains Motivation}
Both trainees and experts recognized that setting small, achievable goals proved to be an effective strategy for sustaining motivation. Through setting incremental targets rather than focusing on the endpoint, trainees and experts could effectively navigate the initial rut of voice training, while via celebrating small achievements (made achievable through incremental targets), experts could build client self-competence through the plateau of voice training.

\paragraph{Incremental goals as a healthy alternative to end-goals}

Several trainees initially set lower goals () or re-evaluated their goals to define dynamic achievable targets (). P5T used this dynamic-goal technique, starting with an easier goal to avoid disappointment:
\begin{quote}
``I set my expectations low for myself. I was aiming for mostly androgynous until I felt like I could get there, and then I aimed further.'' (P5\_trainee)
\end{quote}
Several experts () encourage this approach, recognizing the importance of setting an incremental target rather than an end-goal. P2E mentioned that she focused on an evolving target built on vocal characteristics rather than an exact end-goal voice as part of voice therapy:
\begin{quote}
``I work together with them to set a target and a lot of times it's an evolving target. Instead of saying well we are here and I want your endpoint to be here, we talk more about characteristics of voices.'' (P2\_expert)
\end{quote}
\paragraph{Focusing on incremental achievements to navigate plateaus}
To help clients navigate the later plateau in progress along the voice training journey, experts often employ strategies to maintain motivation and progress through focusing on clients' incremental achievements (P6E, P2E, ...). Several experts () emphasized the importance of focusing clients in on progress over perfection. P2E explains how focusing on clients' incremental achievements builds a sense of self-competence:
\begin{quote}
``let's look at what's positive. What do you like about what's happening and try to keep coming back to some of those positives [...], like, `hey, look at look at all these different things that you have done. And that means that you can do the rest of these things too.''' (P2\_expert)
\end{quote}
Trainee experiences with success through celebrations of incremental progress echo this pattern. P11T described how using the technique of focusing on voice training a single word and spreading the training to specific consonants and vowels allowed her to see substantial progress through the initial period of voice training:
\begin{quote}
``It's really fun because, wow, I'm making so much progress. I can tell I'm bringing this [phoneme] into line the next day.'' (P11\_trainee)
\end{quote}
Trainee fears around using their voice-in-training (VIT) with others centered fears of their voice not being ready yet (). P6E emphasized highlighting progress in specific voice characteristics while de-emphasizing perfection to allow clients to overcome fears about using their VIT with others:
\begin{quote}
``I know that this doesn't quite feel right [for using with others] yet [...] So giving that encouragement that things are sounding good, or you're doing XY and Z well [...] [is] setting people up for success knowing that sometimes things are not going to be perfect and that's OK.'' (P6\_expert)
\end{quote}
\subsubsection{The Progress-Motivation Cycle}
The perspectives of trainees and experts indicate a strong cyclical relationship between progress and motivation in voice training. Noticeable progress fuels motivation, which in turn drives further progress --- fueling the steep progression curve in the middle of the voice training journey. Conversely, demoralization from noticing the distance from a goal or failing to perceive progress leads to less frequent and effective voice training, both by reducing the drive to engage in voice training practice and by creating psychological barriers to using tools like voice recordings, reducing progress --- exacerbating the initial rut of voice training and the eventual plateau.
\paragraph{Progress makes voice training fun}
Several trainees () mentioned that perceiving progress in their voice made voice training an enjoyable process, as opposed to a chore (). P11T mentioned how her perception of daily progress during a rapid phase of voice training compounded into even more progress:
\begin{quote}
``It was really fun when I could tell I was making a lot of progress every day. That's really fun. That's like, really encouraging. It's like [...] That's why I made so much progress in the last two months of training.'' (P11\_trainee)
\end{quote}
\paragraph{Demoralization leads to inconsistent and less effective voice training}
Conversely, a perceived lack of progress can significantly demotivate trainees. Several trainees () mentioned that realizing how far away they were from their goals caused them to voice train less effectively or frequently. Multiple trainees (mentioned that dysphoria about their voice prevented them from utilizing beneficial voice training tools, such as voice recording or analysis software (P11T...). P11T mentioned that the daily demoralizing impact of realizing this distance from the voice training end-goal prevented her from using voice recordings to check in with her voice:
\begin{quote}
``I could not record my voice because I could tell how far away I am [...] it's very demoralizing to realize every single day how far away I am.'' (P11\_trainee)
\end{quote}
\paragraph{Universal expectations drive negative self-perception}
Experts recognized this challenge and emphasized the importance of acknowledging the unpredictability of voice training results and progress. Several experts () mentioned how voice training media (VTM) can create unrealistic expectations of continuous progress through its one-size-fits-all approach to voice training (). {} mentioned how this expectation of progress driven by VTM can create negative self-perceptions among voice trainees:
%TODO: get the quote here -- it exists, just need to search it
\begin{quote}
    
\end{quote}

\begin{quote}
``And you know, there's a lot of counseling that goes into it of talking about like, `OK, that one experience is not the be all end all. So just because you had one bad experience with it, you know, we'll talk about [...] You know, you do have. You do have some control, but yeah, sometimes it's going to be unpredictable.'' (P2\_expert)
\end{quote}

\subsubsection{Challenges in Voice Generalization and VIT Use}

One of the most significant challenges in voice training is generalizing the trained voice to real-world situations. Many trainees reported difficulties in using their voice-in-training (VIT) in various contexts:

\begin{quote}
``In public would be where I would be training my voice. So anytime that like my voice like broke or like I didn't like [...] I wasn't consistent with it. I would notice and I would be super stressed out about it because then I'd be having this conversation with something I'd be like forgetting what they're saying because I'm so focused on how I sound.'' (P5\_trainee)
\end{quote}

Experts acknowledged these challenges and often provided strategies to facilitate VIT use in various contexts:

\begin{quote}
``Scripting. I really like the idea of scripting, whether it's a coffee order I we talk about anchor words or anchor phrases, so I'll say pick something that you're going to say several times during the week. The things that are most routine, the way that you greet someone, the way that you say goodbye, the way that you [...] Maybe on a colleague or a friend you're checking in on them.'' (P7\_expert)
\end{quote}

\subsubsection{External Barriers and Their Impact on Progress}

External factors, such as health issues or safety concerns, often pose significant challenges to voice training progress. One expert noted:

\begin{quote}
``I mean physical setbacks like getting sick [...] If you get a bad cold or COVID in the middle of voice training, I think that sets [...] People back quite a bit.'' (P2\_expert)
\end{quote}

Workplace concerns and worries about outing themselves as transgender also emerged as a significant factor influencing voice use, as one trainee shared:

\begin{quote}
``Well said, say work. I'm not out and [...] So yeah, sometimes I drop into a professional [...] Male voice and [...] That's just, you know, you got to make a living.'' (P10\_trainee)
\end{quote}

\subsubsection{Vocal Dysphoria: A Barrier to Progress and Tool Utilization}

Vocal dysphoria emerged as a significant barrier to progress and tool utilization in voice training. Many trainees reported that dysphoria prevented them from engaging fully with their training:

\begin{quote}
``Oh, sure. Yeah. Yeah. I mean, I used it. I started 20. I just, like, started 24/7 immediately. And yeah, it was. It was bad for a while. So I would just like not listen to myself ever. I didn't take any recordings of myself, which definitely slowed my progress.'' (P11\_trainee)
\end{quote}

Experts recognized this challenge and emphasized the importance of addressing dysphoria to facilitate progress:

\begin{quote}
``And then I think you know a big the biggest thing is probably just like voice dysphoria and like a lot of people want to work on their voice. But when they start this journey, it it can be too much and sometimes it's not the right time for everyone.'' (P3\_expert)
\end{quote}

\subsubsection{The Delicate Balance of Feedback}

Feedback plays a crucial role in voice training, but our findings reveal the complexity of managing feedback effectively. Experts emphasized the need for grounded, objective feedback:

\begin{quote}
``I try to provide as much feedback as I can, right. And I think I try to provide that coming from a place of like a professional, but also like a personal place, right. Like I thought your voice sounded really good. You know, obviously this is my job. But also like I'm a person and I'm listening to their voice, and I can provide [...] Feedback on that?'' (P4\_expert)
\end{quote}

However, trainees often encountered challenges with overly positive or non-constructive feedback, particularly from their support networks:

\begin{quote}
``And then I don't know if people are indulging me or not, but some people think that I already have a a feminine voice and I think they're pulling my leg.'' (P10\_trainee)
\end{quote}

To address this, experts often encouraged the use of more objective-sounding forms of voice measurement which can be shared with those close to them, such as rating scales:

\begin{quote}
``For a few patients, I've sent home kind of like an arbitrary rating scale, like zero to 10, right? And I work primarily with voice feminization clients [...] Like 0 is very masculine sounding, 10 is very feminine sounding [...] them self rating can be helpful like oh that time it, you know, felt or sounded like a six that time it felt or sounded like an 8 that sort of thing.'' (P4\_expert)
\end{quote}
\subsection{Generalization and Using the Voice-in-Training (VIT)}

Our research highlights the critical importance of voice generalization - the process of transferring newly acquired voice skills to real-world situations. This section explores the strategies and challenges involved in using the Voice-in-Training (VIT) across various contexts.
\subsubsection{Preparing the VIT for Use}

% Paragraph on the importance of warm-up exercises
% Reference: Expert codebook > Practicing Voice > IVT: setting targets to hit throughout the day
% Quote from expert about designing warm-up routines for clients

% Paragraph on trainee experiences with VIT preparation
% Reference: Trainee codebook > IVT Techniques > VIT Maintenance and Recovery in Conversation > Warming up before using VIT (through voice exercises)
% Quote from trainee about their pre-conversation warm-up routine

\subsubsection{Self-Accountability in VIT Use}

% Paragraph on the importance of self-accountability
% Reference: Expert codebook > Practicing Voice > Voice Generalization > VIT Maintenance and Recovery in Conversation
% Quote from expert about teaching clients self-monitoring techniques

% Paragraph on using reminders and cues
% Reference: Trainee codebook > Technologies > Unique uses of technologies > Using AI assistant to reinforce use of feminine voice
% Quote from trainee about using technology-based reminders

% Paragraph on low-tech accountability methods
% Reference: Expert codebook > Technology  Practices > Out-of-session > Reminders > using post-its as visual/physical reminders
% Quote from expert about recommending visual cues like post-it notes

\subsubsection{Recovering the VIT During Use}

% Paragraph on techniques for voice resets
% Reference: Expert codebook > Practicing Voice > Voice Generalization > VIT Maintenance and Recovery in Conversation
% Quote from expert about teaching filler/anchor word techniques

% Paragraph on contrast training for voice recovery
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Voice Generalization Exercises > self-perception: negative / contrast practice improves perception of voice
% Quote from expert about the benefits of contrast training

% Paragraph on context-dependent recovery strategies
% Reference: Trainee codebook > IVT Techniques > Social Context and VIT-use > Context impact on IVT and VIT use
% Quote from trainee about their experiences recovering their VIT in different social contexts

\subsubsection{Generalization Exercises for Pre-VIT Use}

% Paragraph on bringing real-life elements into training
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Voice Generalization Exercises > Generalization strategies: importance of authentic practice
% Quote from expert about incorporating client-specific materials into sessions

% Paragraph on scripting techniques
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Voice Generalization Exercises > Scripting
% Quote from expert about using scripting to prepare for common scenarios

% Paragraph on practicing task-specific language
% Reference: Trainee codebook > IVT Techniques > Conversational Targets > Sustain-based targets
% Quote from trainee about practicing work-related terminology

\subsubsection{Gradual Expansion of VIT Use}

% Paragraph on the hierarchy of VIT use contexts
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Practice Environments and Activities > Generalization strategies: working through heirarchy of stressful environments
% Quote from expert about guiding clients through increasingly challenging situations

% Paragraph on trainee experiences with expanding VIT use
% Reference: Trainee codebook > IVT Techniques > Social Context and VIT-use > Working through hierarchy of social contexts when using VIT
% Quote from trainee about their journey from using VIT with close friends to using it in professional settings

\subsubsection{Leveraging Technology and Online Spaces for VIT Practice}

% Paragraph on using online gaming for VIT practice
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Practice Environments and Activities > Generalization strategies: using voice in a game
% Quote from expert about recommending online gaming for voice practice

% Paragraph on trainee experiences with online VIT use
% Reference: Trainee codebook > Technologies > Online Social Spaces > Using online spaces to discuss voice training and voice train with other trans people
% Quote from trainee about using Discord or VRChat for voice practice
\subsection{Technologies in Voice Training: Current Use and Future Directions}

Our research revealed a complex landscape of technology use in voice training, with both experts and trainees leveraging various tools to support the training process. This section explores current technology use, attitudes towards these technologies, and their social impacts on the voice training journey.
\subsubsection{Responsible Use of Voice Training Technologies}

Both experts and trainees emphasized the importance of using voice training technologies responsibly to avoid potential pitfalls.

% Paragraph on avoiding perfectionism with measurement tools
% Reference: Expert codebook > Technology  Practices > Problems with technologies > Overuse of pitch grabber creates perfectionism
% Reference: Trainee codebook > Technologies > Voice Tools/Pitch Grabbers > (Too much) emphasis on pitch
% Quote from expert about the dangers of over-reliance on pitch measurements
% Quote from trainee about their experience with perfectionism when using pitch grabbers

% Paragraph on the importance of trainee-set targets
% Reference: Expert codebook > Client Goals > Approximate Goals > How Clients Describe Goals
% Reference: Trainee codebook > Technologies > Voice Tools/Pitch Grabbers > Voice tools did not capture my needs well
% Quote from expert about guiding clients to set their own realistic targets
% Quote from trainee about the mismatch between technology-set targets and personal goals

% Paragraph on the multi-faceted nature of voice beyond pitch
% Reference: Expert codebook > SLP Strategies > Skill-building > understanding parameters
% Reference: Trainee codebook > voice goals > Factors that influence goals > Focus on Parameters/Techniques
% Quote from expert about teaching clients about various voice parameters
% Quote from trainee about their realization that pitch alone doesn't determine voice gender
\subsubsection{Technologies as a Medium for Human Interaction}

% Paragraph on teletherapy use by experts
% Reference: Expert codebook > Demographics > Type of session > mostly work through teletherapy
% Quote from expert about their experience with teletherapy

% Paragraph on online communities for trainee interaction
% Reference: Trainee codebook > Technologies > Online Social Spaces > Using online spaces to discuss voice training and voice train with other trans people
% Quote from trainee about their experience in online voice training communities

% Paragraph on potential for online support networks for voice training from an expert-perspective
% Reference: Trainee codebook > Technologies > Online Social Spaces
% Reference: Expert codebook > Ideal Technologies > Brainstorming: want easier way to connect with online support group
% Quote from trainee about their experience in online voice training communities
% Quote from expert about the potential of online support networks


\subsubsection{Positive Impacts of Social Technologies on Voice Training}

% Paragraph on support communities
% Reference: Trainee codebook > Voice training techniques > Social Influences on Voice Training > Social feedback
% Reference: Expert codebook > Support Networks
% Quote from trainee about receiving tailored feedback from peers
% Quote from expert about the benefits of peer support networks

% Paragraph on voice training media (VTM) as an educational resource
% Reference: Trainee codebook > Technologies > Voice Training Media (VTM) > how VTM is used > VTM for building knowledge
% Reference: Expert codebook > Technology  Practices > Out-of-session > Voice Training Media (VTM)
% Quote from trainee about learning voice training methodologies through online resources
% Quote from expert about recommending specific VTM resources to clients

% Paragraph on VTM overcoming financial barriers
% Reference: Trainee codebook > Voice Training Challenges > Other challenges/barriers > Pain-points: finding accessible (financially) resources for voice training
% Quote from trainee about using free online resources due to financial constraints

\subsubsection{Potential Negative Impacts of Social Technologies}

% Paragraph on overgeneralized voice training media
% Reference: Expert codebook > Technology  Practices > Problems with technologies > Need for Responsible Technology Use
% Quote from expert about the dangers of one-size-fits-all voice training advice

% Paragraph on unrealistic standards created by VTM and online communities
% Reference: Trainee codebook > Technologies > Voice Training Media (VTM) > "Standard of ""beauty"""
% Quote from trainee about feeling pressured by online voice standards

% Paragraph on the "diet culture" effect in voice training communities
% Reference: Trainee codebook > Technologies > Voice Training Media (VTM) > "Standard of ""beauty""" > VTM creating a specific voice culture standard for voice training is a negative thing
% Reference: Expert codebook > Client Goals > Clear Goals > Problems with Clear/Rigid Goals
% Quote from trainee about the pressure to achieve a certain type of voice
% Quote from expert about helping clients set realistic, individualized goals
\subsubsection{Unique and Repurposed Technologies for Voice Training}

% Paragraph on non-traditional voice training tools
% Reference: Trainee codebook > Technologies > Unique uses of technologies
% Reference: Expert codebook > Technology  Practices > In-session > using LLMs for generating reading samples
% Quote from trainee about using a non-voice-specific app for training
% Quote from expert about creative use of technology in sessions

% Paragraph on repurposing gaming and social platforms for voice practice
% Reference: Trainee codebook > Technologies > Online Social Spaces > Using online spaces to discuss voice training and voice train with other trans people
% Reference: Expert codebook > Practicing Voice > Voice Generalization > Practice Environments and Activities > Accessible/Low-cognition tasks
% Quote from trainee about using gaming platforms for voice practice
% Quote from expert about recommending low-stress online environments for practice

% Paragraph on voice changer use and perceptions
% Reference: Trainee codebook > Technologies > Voice changers > Voice changer potential for goal exploration / testing voices
% Reference: Expert codebook > Brainstorming > Simulated Environments for Voice Generalization (SEVG) > voice changers
% Quote from trainee about using voice changers for goal exploration
% Quote from expert about the potential benefits and risks of voice changer technology



==> extra_files/old_versions/old_methods.tex <==
%TODO: Update tables with missing information
%TODO: Update mean / standard deviation, and ranges since determined pilots after some of these were calculated
%TODO: Write Positionality Statement (with identities of the three researchers)
%TODO: WAIT UNTIL LAST EDIT: fix participant numbering starting with lowest-number participant.
%   - For trainees, go two down (P3T->P1T)
%   - For experts, go one down (P2E->P1E)
To better understand how voice goals, voice practice methods, and voice generalization strategies interact with technology use, we conducted an interview study involving gender-affirming voice experts and voice trainees with at least three months of voice training experience.

\subsection{Participants}
We recruited two groups of participants, 6 gender-affirming voice experts, including 5 Speech-Language Pathologists (SLPs) and one SLP-in-training, and ten voice trainees, comprising transgender individuals at various stages of their voice training journeys.

% Additionally, we conducted pilot interviews with one voice coach (expert) and two voice trainees. While we do not include data from these pilot interviews in the main analysis, we used them to refine the interview scripts and develop the brainstorming section.

%Recruitment was conducted through online forums, voice training communities, university-wide research recruitment emails, and other universities with gender-affirming voice specialists. All participants were located in the United States, and all interviews were conducted in English. Participants were compensated at a rate of \$25/hour upon completion of the study.

\subsubsection{Voice Experts}
%Describe recruitment method here
We recruited 6 voice experts, with ages ranging from 27 to 47 (\textit{M} = 32.5, \textit{SD} = 7.56) and years of experience ranging from 2.5 to 18 (\textit{M} = 7.25, \textit{SD} = 5.44). Among the voice experts, two (P3E, P7E) identified as transgender and/or nonbinary, one (P6E) was a cisgender man, and three (P2E, P4E, P5E) were cisgender women. Table \ref{tab:expert_demographics} shows voice experts' demographic information.

We emailed expert recruitment information to gender-affirming voice therapy programs at various universities and through our own university's research email recruitment system. To be eligible for participation, voice experts had to be at least 18 years old and have experience conducting gender-affirming voice therapy or coaching with transgender clients.

\begin{table}[h]
\caption{Voice Expert Demographics \yuhang{the current numbering method is a little hard to track... maybe use P1-P10 for trainees, and E1-E6 for experts.}}
\label{tab:expert_demographics}
\begin{tabular}{cccccc}
\hline
Participant & Transgender? & Gender-Nonconforming? & Gender Identity & Age & Years of Experience \\
\hline
P2E & No & No & Female & 47 & 18 \\
P3E & Yes & Yes & Nonbinary & 30 & 3 \\
P4E & No & No & Female & 33 & 9 \\
P5E & No & No & Female & 23 & 3 \\
P6E & No & No & Male & 27 & 2.5 \\
P7E & Yes & Yes & Nonbinary & 35 & 8 \\
\hline
\end{tabular}
\end{table}

\subsubsection{Voice Trainees}
%Describe recruitment method here
We recruited ten voice trainee participants (excluding the pilots) with ages ranging from 19 to 68 (\textit{M} = 31.3, \textit{SD} = 13.88). The trainees represented a diverse range of gender identities and voice training goals, including masculinization, feminization, and androgenization. The group comprised one (P3T) nonbinary transfeminine participant, one (P8T) nonbinary transmasculine participant, six trans women (P5T-P7T, P9T-P11T), and two trans men. P4T and P12T noted that testosterone-based hormone therapy had lowered their voices, while P8T mentioned that they were not on testosterone. P5T mentioned that she started puberty blockers before adulthood, but already had her voice drop because of testosterone-based puberty. Both P4T and P12T are bilingual, with experiences that reflect voice training in two languages. Participants had varying levels of voice training experience, with some independently working on voice training and others working with voice experts such as voice coaches or SLPs. Table \ref{tab:trainee_demographics} shows voice trainees' demographic information.

We emailed trainee recruitment information through our university's research email recruitment system and created recruitment postings on multiple transgender identity-focused and voice training-focused Discord servers. Participants were eligible if they were at least 18 years old and had at least three months of consistent gender-affirming voice training experience, either alongside an expert or without an expert. 

\begin{table}[h]
\caption{Voice Trainee Demographics \yuhang{adjust table size... should go beyond the text width}}
\label{tab:trainee_demographics}
\begin{tabular}{cccccc}
\hline
Participant & Age & Gender Identity & Time Voice Training & Progress Estimate & Worked w/ Expert? \\
\hline
P3T & 36 & Nonbinary transfeminine & 2 years & Inconsistent & Yes\\
P4T & 24 & Male & 2-3 years & 75\% through & No\\
P5T & 20 & Female & 3-4 years & Near-done & No\\
P6T & 19 & Female & 3 years & Near-done & No\\
P7T & 25 & Female & 1-2 years & Midway & No\\
P8T & 20 & Nonbinary transmasc & 2 years & Ongoing & No\\
P9T & 38 & Female & 8 months & Near midway & Yes\\
P10T & 68 & Female & 2 years & Ongoing & Yes\\
P11T & 29 & Female & 2 years & Finished & No\\
P12T & 34 & Male & 2 years & Midway & No\\
\hline
\end{tabular}
\end{table}

\subsection{Procedure}
%Motivation first -- why did we recruit two groups of participants
 %and voice trainees via Zoom. Expert interviews lasted 1-1.5 hours, while trainee interviews lasted 1-2 hours. \yuhang{revisit your VR paper for method writing...also avoid one single sentence as a paragraph. You can merge the short paragraphs in procedure. Moreover, i don't think you need to use sections to divide the interviews. Just say, we first ask about xxx, then we asked about xxx. Currently, the sections are divided too thoroughly.}
%motivation first
% \begin{enumerate}
%     \item Demographics
%     \item Base voice training techniques
%     \item Technologies used
%     \item Incorporation of voice training into daily life
%     \item Brainstorming
% \end{enumerate}
%Not bullet point
We conducted 1-1.5 hour single-session interviews with both gender-affirming voice experts via zoom. We first gathered information about age, gender identity, professional role, and years of experience. Then, we explored clients' initial understanding of their goal voice, techniques and technologies used in the voice discovery process, methods for measuring voice suitability, specific aspects of voice typically trained, and common pain-points in voice training efforts. We then asked experts about the use of voice-training-specific technologies (e.g., pitch analyzers, spectrograms) and more general technologies benefiting voice training (e.g., voice-chat and social VR applications) inside and outside sessions. We then focused on how voice therapists aided clients in generalizing their voice use, transitioning from exercises to using their voice-in-training in social environments. Finally, we brainstormed a voice training system utilizing RVC voice changers and discussed potential features for goal-voice exploration, incremental target setting, and simulated conversation environments using social VR.
% \begin{enumerate}
%     \item Demographics
%     \item Goal voice exploration
%     \item Understanding the voice goal and setting targets
%     \item Social and technological influences on voice goals and targets
%     \item Brainstorming
% \end{enumerate}
%Do not bullet-point

We conducted 1-2 hour single-session interviews with trainees via Zoom. We first gathered information about age, gender identity, voice training experience, and work with voice experts. We then focused on how trainees identified and modified their voice goals, and what factors informed these goals. Next, we examined how voice goals informed training, starting with how the goal impacted their perception of the voice training journey, then identifying how goals shaped their target-setting practices, including voice generalization targets when applicable. We then asked about the social and technological influences on goal and target-setting, including the impact of voice training media and communities, voice changers, and pitch-grabber applications. Finally, we brainstormed a voice training system with the same design as the system from the expert interviews, but asked questions focused on trainees' experiences and desires for voice training technology.
\subsection{Data Recording and Analysis}
%Too thorough -- talk about more generically
%We employed a rigorous, multi-stage thematic analysis approach to analyze the interview data, combining elements of grounded theory with a more structured analytical framework. This process allowed us to remain grounded in the participants' experiences while also identifying overarching themes relevant to our research questions.
All interviews were conducted and recorded by a single researcher using Zoom. We used Zoom's automatic transcription service for transcription. To ensure accuracy, we listened to the audio recordings while coding the transcripts, making corrections to the transcripts as necessary. Throughout the interview process, we made iterative improvements to the brainstorming section of our interviews. We analyzed transcripts using thematic analysis \cite{thematic_analysis}%Put these bullet points into the sentence above
% \begin{enumerate}
%     \item \textbf{Trainee Coding:} Two researchers independently open-coded three representative trainee transcripts. They then collaborated to reconcile their codes and create an initial trainee codebook. To account for the diverse experiences of trainees, one researcher open-coded a fourth trainee transcript to supplement the codebook.
%     \item \textbf{Expert Coding:} Similarly, two researchers independently open-coded two representative expert transcripts. They then worked together to agree on the open codes and create an initial expert codebook, separate from the trainee codebook.
% \end{enumerate}

We selected three representative transcripts from trainees and two representative samples from experts, which two researchers open-coded independently. Then, the two researchers worked together to agree on codes for the open-coded transcripts and agree on two codebooks, one for experts and one for trainees. They then used these refined codebooks alongside continued independent open-coding for the remaining transcripts. To maintain coding congruence, the two researchers regularly checked each other's codes and open-codes and updated the codebooks for trainees and experts. The two researchers then organized codes on trainee and expert affinity diagrams and identified similar categories between the two diagrams. The final trainee codebook contained over 600 codes, while the final expert codebook contained over 350 codes. Analyzing patterns between the two codebooks, we identified eight shared themes relevant to voice goals and three shared themes relevant to brainstorming goal-voice discovery.%(2+3+3%
\subsection{Positionality Statement}
We acknowledge how the intersection of our identities with our roles as researchers influence our work. The primary researcher, a transgender woman, drew on her lived experience to inform the study design, interview approach, and data interpretation. The second researcher, a cisgender woman with an accessibility research background, contributed to coding, analysis, and background research. The third researcher, a cisgender woman with expertise in accessibility research, ensured research quality and rigor.
%\input{sections/positionality_statement}

==> extra_files/old_versions/old_numbering_findings.tex <==
\subsection{What is a Goal?}
\label{sec:findings:what_is_a_goal}
Previous works on voice training technologies failed to define a clear boundary between overall voice end-goals and voice targets. To better separate these two ideas, we define \textit{voice goals} as the overall heading of the voice training journey, which can be a clear point with specific parameters or characteristics, or a rough area defined through approximate voice features. We define \textit{voice targets} as the measures of success used in daily voice practice, which oftentimes are incremental. While some trainees may use voice goals as targets, experts recommend against doing so. Through focusing on voice goals, %we found that trainees and experts had various ways of defining the ideal end-point to voice training. We found that voice goals
we identified two categories of voice goals: \textit{approximate goals}, which represent the driving factors behind voice training, and \textit{clear goals}, which define a precise direction for voice training.

\subsubsection{Approximate Goals.} We found that while trainees typically didn't have the knowledge to verbalize their initial goals in terms of technical vocal parameters, they still had various characteristics in mind defining the direction of their goals. These approximate goals embodied aspects of vocal utility, comfort, identity representation, or basic parameter explanations. While experts sought to clarify these goals through skill and knowledge-building, the technologies trainees used when training independently measured success through approximate goals.

% \textbf{\textit{Types of Approximate Goals}} 
% Trainees defined approximate goals in terms of utility of the voice, such as having a voice that passes (), representation of their identity, such as having a voice that better represents their gender, a need for personal satisfaction with the voice, such as a voice that doesn't cause dysphoria, or basic single-parameter explanations, such as wanting a higher or lower pitch (). 
\textbf{\textit{Vocal Utility.}} Vocal utility plays a key role in defining why a trainee initially pursues voice training. Specifically, we found that trainees wanted a voice that causes others to treat them a specific way, whether that be passing as cisgender (P3T, P5T, P6T, P10-12T and P2E, P4E, P7E), causing some amount of gender confusion (P8T), or presenting authority (P3T, P4T, P12T). For example, P4T desired a voice so masculine that it would make his coworkers who misgendered him look silly. P8T wanted a voice on the threshold, where most of the time they would be gendered as male, but a small percentage of the time they would be gendered as female by others. For multiple trainees, having access to a voice that passed as cisgender, even if they were gender-nonconforming, would allow them to maintain safety in dangerous environments (P4T, P6T).

\textbf{\textit{Comfort in Voice.}} Trainees mentioned alleviation of voice dysphoria or gaining a voice that they feel comfortable with as a major factor driving their voice training (P3T and P11T). Although providing a point to get away from (the current voice), voice dysphoria oftentimes didn't provide a very useful motivation --- instead, experts recognized voice dysphoria as a common barrier to voice training (P2E, P3E, P5E, P6E), especially when related to \textit{voice generalization}, which involves using the voice-in-training (VIT) in new environments (P2E, P5E, P6E). P2E mentioned how voice dysphoria was a common barrier to practicing outside the session: \textit{``[They're] going home to practice, and if what comes out isn't euphoric, it can be ... a barrier to practicing at all.''} %\yuhang{quote?}%Experts

\textbf{\textit{Identity Representation.}} Identity representation through voice plays a key factor in individualizing the voice goal, providing a vague direction for voice training. Based on the experiences of trainees and experts, we found that identity-based descriptions provided different tiers of specificity. By definition, gender-affirming voice trainees seek to acquire a voice that is affirming for representing their gender identities (P4E, P5E, P6E, P7E). More specifically, some trainees may desire to have a voice that represents their culture or region (P4T and P12T). Voice archetypes and character descriptions, such as ``pretty boy'' (P12T), provided the most detailed representations of approximate goals, since they can be easily connected to examples (P2E, P3E, P6E, P7E). P3E remembered how a character described by a trainee gave her a clear idea of the voice that the trainee wanted:
\begin{quote}
    \textit{``I had one client who said that their ideal voice would be someone who could rock a ball gown but then get in a fight in a bodega. It's a very clear character of what she wanted to sound like.''}
\end{quote}

\textbf{\textit{Parameter-based Goals.}} Trainees with a general knowledge of voice may start with an end-goal focused on shifting specific parameters or aspects (P3T, P4T, P6T, P8T, P11T and P5E, P7E). While providing direction for voice training, this kind of approximate goal may arise from a misconception of the importance of the single parameter, which is usually pitch (P7T and P11T). Experts build a healthy understanding of voice parameters among trainees, allowing trainees to better leverage parameters for approximating their voice goals (P2E-P4E, P5E, P7E)

\textbf{\textit{Approximate Goals in Voice Technologies.}} Voice training technologies like voice tools \cite{voice_tools} used gender-range-based voice targets to attach the approximate goal of presenting gender identity through voice to specific pitch ranges. Trainees and experts lamented that this consistent categorization of voice based on pitch characteristics not only misleads trainees through over-emphasizing pitch (P5T, P7T, P9T-P11T and P2E-P4E, P6E), but also creates unsustainable targets for practice by failing to separate target-setting from goal-setting (P3T, P7T, P11T, P12T and P2E, P3E, P5E, P7E).

\textbf{\textit{Approximate Goals in Voice Training Media.}} While voice training media is a helpful tool for building voice training skills, the untargeted nature of media results in it pushing ideal voice ``standards'' that don't necessarily align with trainees' identities (P3T, P10T, P11T, P12T). P11T developed a Californian ``valley girl'' accent because of the vowel training methods she learned from YouTube, resulting in others mis-identifying her as Californian. P3T described this ``industry-standard'' voice for transfemme individuals:
\begin{quote}
     \textit{``I'm not going to keep pursuing... the industry standard of `We're going to make you sound like you're AFAB. We're going to make you sound like you're 16'.''}
\end{quote}
\subsubsection{Clear Goals.} \yuhang{the first couple of sentences read a bit like background. However, these are your findings, and you identified and defined the concept of these types of goals via your findings. Make sure that you convey that in the writing. For example, at the beginning of5.1, you can say that we identified various types of goals, including xx, xx, used by trainees or experts to achieve xxx. Or at least, to highlight something is your finding instead of some clinical background, you should say "we found that xx."}
Clear goals represent an exact direction for voice training (P2E-P4E, P6E, P7E) through providing a combination of voice characteristics for a trainee to work toward. These goals allow experts to craft individualized training regimens and provide a clearer representation of goal characteristics to voice trainees than approximate goals (P3E, P6E, P7E). We found that experts and trainees triangulate clear goals through combinations of examples and approximate goals, setting a clear direction for voice training.

\textbf{\textit{Example-based Goals.}} Voice examples provided clear goal directions for voice training (P2E-P4E, P2E-P4E, P6E, P7E), as they directly demonstrated voice characteristics which the trainee could work towards. Voice examples used in goal voice exploration came from various aspects of trainees' lives, including people around them (e.g. friends and family) (P3-P5T, P12T and P2E, P3E, P6E), singers, voice actors, and celebrities (P3T, P6T, P7T, P12T and P7E), and online personalities, both transgender (P7T, P11T, P12T) and cisgender (P12T).  Through representing desired vocal characteristics through a single example or multiple examples, experts and trainees could both use examples directly as points of comparison (P2E-P4E) and indirectly through measuring vocal parameters from the example and using them for goal and target-setting (P2E-P4E, P6E, P7E).

\textbf{\textit{Combined Approximate Goals}} While singular approximate goals provide vague direction for voice goals, the combined approximation of multiple vague goals can provide a clear direction for voice training, especially with the guidance of an expert (P9T, P10T and P2E-P4E, P5E, P7E). For independent trainees, voice training resources like Sumian Voice \cite{sumian_voice_examples} provide a (small but growing) database of voices alongside rough character and parameter descriptions which can guide approximate goals to clear goals (P2E, P6E). P3E likened the experience of finding a clear goal to putting together an outfit:
\begin{quote}
\textit{``I use this analogy of going to a clothing store and trying on different pieces of an outfit and piercing it together. So we're trying on different resonance qualities. We're trying on different pitch centers, different articulation styles... And then kind of piercing together their goal voice.''}
%Extra sections if I have time: "Goals are not targets!" and "Multiple Goals"
\end{quote}
\subsection{Characteristics of Goal Exploration.}
\label{sec:findings:characteristics_of_voice_exploration}
While trainees usually begin with approximate goals when starting voice training, the exact direction provided by clear goals allows for more exact voice practice (P2E-P4E). We define \textit{goal exploration} as the process through which trainees and experts arrive at clear goals through exploration. We found that effective goal exploration accounted for the dynamic nature of goals through continuous reevaluation and benefited from voice models as examples who could demonstrate a range of voices. Furthermore, we identified rigid goals as barriers to the voice training journey and de-emphasis of the goal as a necessary step during troughs and plateaus of progress associated with skill-building and voice generalization.

\subsubsection{Goals Change.}
While a major focus of goal voice exploration is finding a voice ``end''-goal, voice training goals are hardly ever static. Instead, they dynamically evolve as trainees build new skills, discover new aspects of their identity, and perceive the changing qualities of their voices. Experts and trainees continue reevaluating goals throughout the voice training journey to maintain a goal that represents the trainees' voice needs.

\textbf{\textit{Why Goals Change.}} The suitability of a goal depends on both factors inherent to voice training (e.g. motivation, skill, knowledge, and voice physiology) (P5T-P7T, P9T, P11T, and all experts) and other personal factors (e.g. identity and environment). As trainees develop their skills and knowledge, their understanding of what is achievable expands (P5E, P6E, P7E). This awareness leads to a recalibration of goals, as trainees pursue more ambitious or nuanced voice characteristics. The effort a trainee invests in voice training is linked to their motivation, which changes throughout the training journey (P6T, P10T, P11T and P3E, P7E). Progress often serves as a powerful motivator, encouraging trainees to set more challenging goals (P11T). Conversely, periods of perceived stagnation may lead to a reevaluation of goals, resulting in more realistic or achievable goals (P11T, P12T and P2E, P3E). As trainees develop their identity, trainees shift their goals to align with their evolving sense of self (P3T, P6T, P9T, P12T). Changes in a trainee's environment (e.g. work or living situation) can necessitate adjustments to voice goals or require trainees to maintain multiple context-dependent goals (P3T, P4T, P7T-P12T and P2E, P3E, P6E, P7E).

\textbf{\textit{Continuous Reevaluation.}} Voice experts emphasize the importance of reevaluating client satisfaction and well-being throughout the goal-setting and training process. Rather than imposing specific targets, most of the experts (all but P5E) emphasized the need to check in regularly on clients' personal comfort and satisfaction with their voices. All experts mentioned that they regularly employed subjective satisfaction-measurement techniques, such as surveys at the beginning of each session. This technique not only gave clients agency in exploration of voice goals, but also allowed for dynamic goal-setting that accommodated for skill and knowledge development among clients (P7E), increasing range with exercising the vocal muscles (P2E, P3E, P7E), and other factors that changed clients' goals, such as changes in overall transition goals (P3E, P6E, P7E).
% \begin{quote}
% ``I work together with them to set a target and a lot of times it's an evolving target. Instead of saying well we are here and I want your endpoint to be here, we talk more about characteristics of voices.'' (P2\_expert)
% \end{quote}
%TODO: new quote from expert here
This approach allows for flexibility in goal-setting and acknowledges the individual nature of voice goals. Trainees (P3T-P6T) also recognized the importance of personal satisfaction with the goal as other factors changed through the voice training journey, often adjusting their goals as they progressed. For P4T and P12T, the impacts of testosterone allowed them to focus less on goals, instead appreciating the progress and forming their voices around the natural changes. P3T shared that their voice goals changed with their personal relationship with voice:
\begin{quote}
``[M]aybe that was an achievable goal, but it wasn't really what I wanted anymore. And my goals sort of shifted to having more acceptance with my voice, whatever that means in any form.''
\end{quote}

\subsubsection{What Makes a Good Voice Example?}
\ref{sec:findings:characteristics_of_voice_exploration:what_makes_a_good_example}
We asked trainees and experts about the types of examples that they used as part of the goal exploration process. For trainees who had examples playing a key role in their goal exploration, the best voice models were people who had a set of voices and flexible range, rather than a single voice, as these models demonstrated the ability to change voice. For voice experts, using examples that demonstrated the full variability of voice allowed them to deconstruct clients' negative perceptions about their voices and shift understanding to the voice as a moldable ``instrument'' (P4E, P6E, P7E). Examples grounded in the trainee's identity, such as other trans people and examples produced through modifications of the trainee's voice, provided clarity to the voice training journey. Furthermore, both trainees and experts recognized the power of centering voice exploration around activities where mimicry is already accepted, such as voice acting or singing.

%Voice actors
\textbf{\textit{Voice Actors.}} Voice actors, who could produce a diverse set of voices from a single vocal ``instrument'', aided trainees in understanding the flexibility of voice (P7T, P12T and P7E). For P7T, the ability of voice actors to produce new voices through minor alterations in various vocal parameters (e.g. pitch, resonance, fry) provided her with a starting point for understanding how these parameters could impact her voice. Experts found that using the framing of voice acting characters, such as in role-playing environments like DnD, afforded trainees more comfort in trying out new voices (P2E, P6E, P7E). P7E found that briefly ``trying on'' voices in-session through approximating the voices of various characters from media helped trainees develop direction to a voice goal.
%Singing
%Singing-training and gender-affirming voice training methodologies are interconnected, as both involve increasing vocal ranges and building skill in managing the fluctuation of vocal characteristics through methods such as vibrato or intonation.

\textbf{\textit{Singers.}} Three trainees found that among voice examples, singers were the most effective for their goal voice exploration (P4T, P11T, P12T). Singing provided a route for trying out voices that didn't have the same baggage as mimicking other voice examples (P11T, P12T). For P4T, mariachi singers provided culturally relevant examples of voices that he could mimic, since he didn't hang around too many Spanish-speaking friends. For P11T, the range and flexibility of singing helped her find voice examples in her accessible range, allowing her to immediately use them for training and break through the psychological barriers preventing her from training, \textit{``My goal for the first several months was just to not bee miserable with it, and so, [for] most of the earlier training, [I] was just singing in the shower.''}

\textbf{\textit{Other Trans People.}} For trainees with unclear journeys to their goal voice, examples of how transgender people changed their voices, such as those available through voice training media like TransVoiceLessons on YouTube \cite{transvoicelessons_youtube} and the trans community around them (P4T, P7T) demonstrated the timeframe that they could expect for voice training, while also giving them an idea of what their voice would sound like throughout the journey. Given trainees' difficulty in estimating the length of the voice journey (P5T, P7T, P9T-P12T), with many trainees feeling reaching a goal voice was impossible (P3T-P5T, P7T, P10T-P12T), these examples of successful voice training allowed trainees to more aggressively set their end-goals (P7T).

\textbf{\textit{My(modified)self.}} While not always providing natural-sounding voices, basic voice changer technologies --- such as voice filters, desktop applications, and advanced vocal processors --- provided inspiration for voice training through examples grounded in trainees' own voices (P3T, P5T, P6T, P8T, P9T, P11T, P12T). We found that the impact of voice changer technologies on goal exploration varied with the effectiveness of the software in producing a natural-sounding voice and the technical knowledge of trainees in navigating difficult interfaces for producing a voice. For trainees with imperfect experiences with voice changers, the goal could still provide a direction to work towards (P3T, P6T, P10T), and an understanding of the limitations of shifting single characteristics of voice (P11T), or specific characteristics to assimilate into their own voices (P3T, P8T). When voice changers performed to provide adequate voices that allowed trainees to present their identities, trainees felt that the voice changer voice unearthed their own potential, as it demonstrated what voice training could do for them (P3T, P12T). For P3T, positive reactions from others to the modified voice increased internalization, functioning as a motivation for voice training:
\begin{quote}
    \textit{``I did produce something that I think was a very passable cis woman's voice. And I remember sharing that with people and them being like, `I can't believe that was you'... I think I really internalized that people are responding with the sort of shock or disbelief that that could even have been me. And that's the response I want.''}
\end{quote}
\subsubsection{Rigidity Around Goals Stalls Voice Training}
While clear goals provide direction to voice training, rigidity around voice goals serves as a potential barrier, especially during the early skill-building and later voice generalization phases of voice training. To combat goal rigidity, experts reduce focus on the voice goal and emphasize incremental targets and progress.

\textbf{\textit{Rigidity Around Unsustainable Goals}} Experts noted that trainees were often set on unsustainable or unsuitable voice goals, especially early in the voice training journey (P2E-P4E, P6E, P7E). These unsustainable goals resulted in trainees straining their voices through unhealthy practice (P3T, P7T, P9T, P12T and P2E, P4E, P6E) while also demoralizing trainees because of the distance to the goals (P10T, P11T and P4E). While experts worked with clients to help them understand voice limitations in relation to the goal (P3E, P4E, P6E), this practice could demotivate trainees while also not representing the plasticity of voice. As an alternative strategy, experts temporarily de-emphasize the goal voice while focusing on incremental targets (P2E, P3E). P3E mentions how they use this technique:
\begin{quote}
    \textit{``I feel like it can start a shame spiral with some people, like `I'm so far away from this goal voice or this person's voice that I was listening to' ... I think in the beginning we might establish, OK, here's where you're starting, [here's where your] fundamental frequency is, and here's where this person that you were listening to is speaking.''}
\end{quote}
 %Include quote here from an expert

\textbf{\textit{The Perfectionist ``Plateau''.}} Voice experts and trainees identified a ``plateau'' to voice training progress following a phase of rapid voice development (P6T, P11T and P2E, P4E). This plateau involved a combination of ``fine-tuning'' work (P6T and P4E) and hurdles for voice generalization (P2E, P3E, P7E). As P6T explained, \textit{``Voice training has a really weird learning curve where you start off [and] you don't see a lot of progress and then there's a period where you're like, `oh, I get it now' and then [for] that month you're gonna get a lot of progress and then later on it's a lot of fine-tuning.''} Trainees  struggled with using an imperfect voice-in-training (VIT) outside controlled practice environments when they thought it wouldn't be perfect (P3T, P5T, P7T, P8T, P10T and P6E, P7E). To combat fears around generalization, trainees controlled the contexts where they would use the VIT (P3T, P4T, P7T, P8T, P11T and all experts) and all experts recommended starting with practice partners that the trainee felt comfortable with. Furthermore, experts (P2E, P5E, P6E, P7E) identified that feedback focused on small achievements could build trainee self-confidence in generalizing their VIT. For example, P6E's encouragement focused on specific voice characteristics, \textit{``[G]iving that encouragement that things are sounding good, or you're doing XY and Z well ... [is] setting people up for success knowing that sometimes things are not going to be perfect and that's OK.''}

%TODO: This section actually builds into setting targets -- return to it if I have time to include targets (and if it doesn't impact the scope too much)
% \subsubsection{Identifying Specific Needs}
% Trainees come from a variety of backgrounds, which not only inform the voice goal itself, but also the techniques for goal voice exploration. Trainees and experts identified how various aspects about the trainee and their environment influenced the goal exploration and target-setting process.

% \textbf{\textit{``Toolbox'' of voices}}
% %Focus on trainees

% \textbf{\textit{Accommodating Various Abilities.}} 
% %Focus on experts

% \textbf{\textit{Leveraging Existing Skills.}}
%Focus on trainees and experts


% ``Yeah, sometimes there might be really good examples of like, I really like looking at like voice actors, for example, who might do a lot of different things and show different parameters of their voice.'' (P7\_trainee)
% \end{quote}
%\textbf{\textit{What the example should do}} 
% \textbf{\textit{Examples for Direction}} Given the distance of examples from trainees' current voices at the start of voice training, several experts () recommended against using an example voice as a target for emulation. P4E described her usage of examples as direction-focused, rather than mimicry-focused:
% \begin{quote}
% ``I tend to have the patient talk about what aspects of that person's voice they like or what things that they are trying to work towards instead of trying to emulate that voice in particular.'' (P4\_expert)
% \end{quote}
%\paragraph{Passing as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention of the "diet culture" and "standard of beauty for voice training and how this influences goals around passing
%Mention of how passing is a social-feedback-based goal, and still exists when a clear goal is set, as it functions as a reliable indicator for some trans individuals of 1) whether they are hitting their targets and 2) whether a clear voice goal is sufficient
%\paragraph{Identity representation as a goal}
%Mention trainees and experts who mentioned this as a goal
%How this is as opposed to passing -- represents both gender-conforming and nonconforming identities, while representing other qualities of identity as well, such as culture
%How this guides into clear goals, such as finding examples that match one's identity (culture, accent, age, gender)
%\paragraph{Overcoming voice dysphoria as a goal}
%Mention trainees and experts who mentioned this as a goal
%Mention how voice dysphoria can be both a driving factor and barrier to trainees pursuing voice training
%Mention how trainees and experts use comfort with a voice as a factor when transforming the vague goal of overcoming voice dysphoria to clear evaluations of examples for voice goals
%\paragraph{Changing pitch as a goal}
%Mention of how trainees regularly start with vague ideas of what voice training is and the qualities of voice -- from both the experiences of experts with clients and trainees' perspectives
%Mention how voice training technologies, such as pitch-grabbers like voice tools (with pitch as the guidance factor for being "on-target" with a gender), and basic gender-based voice changers (which change only pitch) misinform trainees on the importance of pitch as a factor to "passing" or sounding like they want to sound -- but also how some trainees found that these tools helped them come to this understanding
%Mention how this builds into clear goals, both through:
%1) Developing a clearer knowledge of the limitations of a pitch and the need to include other parameters like resonance and weight
%2) The single parameter being a possible guiding factor for finding voice examples which capture further aspects of voice
% \subsubsection{Models guiding the goal}
% When discussing goal exploration methodology, both trainees and experts mentioned voice-parameter-driven ( and ) and example-driven ( and ) methods for exploring voice goals, alongside methods that used voice examples for demonstrating voice parameters ( and ). 
% \paragraph{Finding voice examples}
% %mention resources where trainees find models including the internet (e.g. Voice Training Media, Singers, Friends online, Youtubers) and the importance to trainees of finding models that match their voice characteristics
% \paragraph{Expert experiences using models to find goal voice}
% %mention how experts find that clients bring in models for how they want to sound, both prompted and unprompted
% \paragraph{Who to model?}
% %mention the types of models that trainees / experts bring in
% \paragraph{Issues of voice ownership and mimicry}
% %mention that copying a model can make voice feel like an impression for trainees -> low sense of ownership
% \subsubsection{Perspectives on Clear Goals}
% \paragraph{Making the expert's job easier}
% %Various points to go over that various experts mentioned -- makes understanding the parameters and voice exercises easier, makes
% \paragraph{The Pitfall of Rigid Goals}
% %expert perspective -- deadset on rigid goals creates perfectionism and loss of motivation
% %trainee perspective -- setting a goal that is too difficul to reach
% \subsubsection{Examples as goal approximation tools}
% Several trainees and experts ( and ) found that a responsible use of voice examples in goal voice exploration involved treating the models not as goals, but instead as both targets to approximate ( and ) and instruments to pull qualities from ( and ).
% \paragraph{Example approximation for goal discovery}
% \paragraph{Extracting vocal qualities from examples}
% \paragraph{Facilitating a responsible understanding of examples}
% %START OF GVD SECTION
% %NOTE: should "brainstorming" subsections like this be moved to the end of the findings section and included in a separate section? -- in which case would it be fine to include references to previous findings sections?
% \subsubsection{Examples as goal approximation tools}
% Several trainees and experts ( and ) found that a responsible use of voice examples in goal voice exploration involved treating the models not as goals, but instead as both targets to approximate ( and ) and instruments to pull qualities from ( and ).
% \paragraph{Example approximation for goal discovery}
% \paragraph{Extracting vocal qualities from examples}
% \paragraph{Facilitating a responsible understanding of examples}
%START OF GVD SECTION
%NOTE: should "brainstorming" subsections like this be moved to the end of the findings section and included in a separate section? -- in which case would it be fine to include references to previous findings sections?
\subsection{Towards a Goal-Voice-Discovery Tool}
\label{sec:findings:towards_a_goal_voice_discovery_tool}
As part of trainee and expert brainstorming, we asked questions related to software-development of a voiced training tool for discovering voice goals, which we named the Goal-Voice-Discovery (GVD) tool. As part of this tool, we would create a large dataset of voice examples using Retrieval-based Voice Conversion (RVC) technology. Based on the interviews, we identified several factors important to voice trainees and voice experts for the use of examples in goal voice exploration, including a need for a diverse range of examples representing various gender identities, cultural identities, ages, and voice archetypes, a way to create a voice goal that voice trainees can foster ownership over as opposed to an impression of someone else, and a flexible approach to understanding examples that guides approximation instead of rigid perfectionism. To address these factors in the context of the GVD tool, we brainstormed various features alongside voice trainees and experts. 

\subsubsection{Filtering and Arranging a Voice Database.}
Voice trainees and experts emphasized the need for a large database of voice models, including various gender, cultural, and age characteristics (P5T, P8T, P9T, P11T, P12T and P4E, P5E, P6E). Our research team recognized the need for methods to search, arrange, and filter through such a large database. Methods for filtering, arranging and searching through the voice database included (1) measurable-parameter based methods and (2) model tagging systems requiring human intervention. 

\textbf{\textit{Parameter-based Methods.}} Among parameter-based methods, several techniques emerged, including allowing trainees to define ranges for various vocal parameters including pitch, resonance, and intonation (P4T-P9T, P11T), using voice-analysis techniques such as pitch range measurement to automatically determine a set of goals feasible and suitable for the trainee (P3T, P8T-P12T), and allowing trainees to edit parameters directly using a parameter-based voice changer (not RVC) to see what sounds good, either based on their current voice or a voice example (P3T).

\textbf{\textit{Tagging Methods.}} Among human-description-based tagging methods, desired voice features included voice accent, such as a valley girl or midwestern accent (P5T, P9T, P10T, P11T and P6E), voice archetypes, such as an authoritative feminine voice or a ``pretty boy'' voice (P12T and P4E, P7E), features of voice not yet directly measurable by voice-analysis software, including breathiness, brightness, and scratchiness (P8T, P9T and P4E, P5E, P6E), and characteristics of the person who the model is based on, including emotional characteristics, age and gender (P10T, P12T). To manage tagging of a large database while also giving trainees agency to describe voices using characteristics understandable to themselves, P7E recommended crowdsourcing methods for voice-tagging, such as those employed by the voice training website Sumian Voice \cite{sumian_voice_wiki}.

\subsubsection{Creating Grounded and Unique Voices.} While full-conversion voice changers provided voices representing various identities, trainees worried directly using another person's voice as a goal would create a low sense of ownership (P3T, P8T), result in a non-unique voice (P9T), or create a voice that was too difficult to achieve (P3T, P4T, P10T and P4E-P6E). To address this, we explored various voice-changer-inspired techniques for creating unique voices.

\textbf{\textit{Merging Models.}} In brainstorming the use of this technology as it applies to the problem of voice ownership and individualized voice goals, two use-cases emerged for RVC-model merging. The first was merging multiple voice models together from the database to create unique voices that didn't exist before (P7T). The second was creating a model of the trainee's current voice and merging it with the desired model to maintain voice characteristics, grounding the goal voice with characteristics from the trainees' original voice (P3T).

\textbf{\textit{Simple Voice Changers.}} We also discussed the use of more basic parameter-based voice changers, with integrations into the GVD system including voice-parameter-based voice changers instead of full-conversion on the trainee's original voice to maximize likeness to the original voice at the cost of the goal model not necessarily sounding natural (P3T, P10T, and P7E). These included using voice-parameter-based voice changers as an extra layer on top of an RVC-based voice changer to allow for further customization in creating a unique voice (P3T, P10T), and pulling understandable parameters from the RVC-based voice changer model to feed a more basic parameter-based voice changer, then modifying the current voice using these parameters to create an approximation that maintains characteristics of the original voice (P3T).

%Maybe work into previous section?
\textbf{\textit{Visualizing the journey to a goal}}
To emphasize the goal as a direction rather than an impression to be perfected, we worked with experts and trainees to determine methods for visualizing the journey towards the goal voice model. Among important features mentioned by trainees and experts were (1) voice parameter measurements of the model, such as pitch, resonance, and pitch range (P3T, P7T, P9T, P11T, P12T and P2E, P5E, P6E, P7E), (2) effort, difficulty, and time approximations representing the current voice's distance from the model (P5T, P8T), and (3) milestone models as ``steps'' to the model (P5T). To understand the current voice's distance from the model, we discussed (1) merging models between the trainee's current voice and the model voice with varying weights, reducing the current voice weight for increments closer to the model (P5T), (2) using voice models that are not directly the end-goal, but currently emulate-able by the trainee for practice in the direction of the goal model (P7T, P10T), and presenting the journey in a gamified way, such as milestones and rewards used in language-learning applications like Duolingo (P3T, P4T, P12T and P7E).

==> extra_files/old_versions/old_related_works.tex <==
% \subsection{Positive Impacts of Gender-Affirming Voice Training}
%First paragraph as an overview

% - Safety (getting gendered appropriately oftentimes means being seen as cisgender, and avoiding the dangers of being seen as transgender in unsafe spaces)
% \paragraph{Safety}
% %People make judgements of someone whithin a second based on their voice, and these judgements include gender judgements [perception_of_gender_based_on_voice_first]. For trans individuals, incorrect judgements of gender based on voice not only create feelings of gender dysphoria, but also pose safety risks when non-congruent with displayed gender characteristics. As with other stigmatized identities, identity management is an important aspect of transgender individuals' experiences when navigating social spaces []. Exposure of transgender gender identity through voice takes away trans individuals' autonomy of identity management, making it difficult for them to 
% People make judgements of someone within a second based on their voice, and these judgements include gender judgements \cite{perception_of_gender_based_on_voice_first}. For trans individuals, incorrect judgements of gender based on voice not only create feelings of gender dysphoria, but also pose safety risks when non-congruent with displayed gender characteristics. As with other stigmatized identities, identity management is an important aspect of transgender individuals' experiences when navigating social spaces \cite{trans_identitiy_development_management_and_affirmation}. Exposure of transgender identity through voice takes away trans individuals' autonomy of identity management, and others' perceptions of them as transgender increases risks of violence and harassment \cite{}. 
% % - Navigating a cisgender world -- make sure to get both sides -- both anti-assimilation and pro
% \paragraph{Navigating a Cis World}

% % - Gender Affirmation and Euphoria -- Having others treat you as you are increases psychological well-being (and maybe mention physical as well)
% \paragraph{Gender Affirmation and Euphoria}

% %Going over voice-training techniques, focusing on research specific to the voice therapy area
% \subsection{Voice-Training Techniques}
% %First paragraph as an overview

% %Basic (Pitch) to more detailed (Pitch + Vocal Tract Length (VTL) to new technologies (ML) for assessing voice gender compared to people's perceptions (irl and through modern survey techniques) -- include Robin's work here
% \paragraph{Gendered Voice Measurement}

% %Focus on the progression of transgender community's use of various technologies and the different kinds of technologies that can benefit voice training, plus new developments in voice training 
% \subsection{Voice-Training Technologies}
% %First paragraph as an overview

% %From the initial voice training VHS to the to the modern Youtube series, alongside text-based media such as trans voice wikis on Reddit
% \paragraph{Voice Training Media}

% %Social media, Discord, VRChat -- voice workshops, transgender people working together, and online voice coaches -- might not fit here since I'm not sure how much research there is in this area?
% \paragraph{Forming Online Communities}

% %Mention academic studies on voice training applications and inclusive design, and also apps available on phones
% \paragraph{An App for Voice Training}

% %Going over voice changers and synthesizers and the various technologies available, how they work when built into accessibility tools, and how transgender people use them for identity representation in social VR spaces -- and the interactions between voice changers and voice training that happens in these spaces (passing with voice changer vs. not passing but also voice changer as a support/crutch/barrier for voice training)
% \subsection{Voice Changers}
% %First paragraph as an overview

% %Voice Changing Technologies including:
% % - basic voice changers that modify properties like pitch (e.g. clownfish, supervoicechanger)
% % - more advance voice changers that use machine learning (e.g. MorphVox)
% % - high-performance voice changers that use "deepfakes" -- AI voice changers like VoiceMod (most heavily used), w-okada (open-source, uses RVC), and new lower-latency models like LLVC (low-latency voice changer, based on RVC, there's a research article on this)
% \paragraph{Voice Changing Technologies}

%Focus on voice changers which allow users to edit various characteristics of the voice, what these characteristics are, and then the problems with how these characteristics do not relate to actual voice training knowledge/SLP definitions of voice qualities -- then reference Robin's perceptual voice paper -- mention how using voice parameters connected to perceptual qualities such as those on CAPE-V leads to easier manipulation of voice for the purpose of voice training
\paragraph{Manual voice changers}

\paragraph{AI voice changers}

% - My previous paper goes here! -- Transgender people using voice changer for gender identity representation in social VR, interactions with voice training, etc.
\paragraph{Voice Changer interactions with Voice Training}
